Towards Non-Parametric Learning to Rank

This paper studies a stylized, yet natural, learning-to-rank problem and points out the critical incorrectness of a widely used nearest neighbor algorithm. We consider a model with $n$ agents (users) $\{x_i\}_{i \in [n]}$ and $m$ alternatives (items) $\{y_j\}_{j \in [m]}$, each of which is associated with a latent feature vector. Agents rank items nondeterministically according to the Plackett-Luce model, where the higher the utility of an item to the agent, the more likely this item will be ranked high by the agent. Our goal is to find neighbors of an arbitrary agent or alternative in the latent space. We first show that the Kendall-tau distance based kNN produces incorrect results in our model. Next, we fix the problem by introducing a new algorithm with features constructed from "global information" of the data matrix. Our approach is in sharp contrast to most existing feature engineering methods. Finally, we design another new algorithm identifying similar alternatives. The construction of alternative features can be done using "local information," highlighting the algorithmic difference between finding similar agents and similar alternatives.

==> backup_old_ao_proof.tex <==
\begin{theorem}For $D_Y = \text{Uniform}[0,1]$ and $x_{n+1}\leq 0.25$, we have,
$$x^* = \arg \min_{x_i} \{\mathbbm{E}_{Y}\left[\nkt(R_{n +1}, R_i)\right]\} = 0$$
for $x_{n+1}\geq 0.75$, we have,
$$x^* = \arg \min_{x_i} \{\mathbbm{E}_{Y}\left[\nkt(R_{n +1}, R_i)\right]\} = 1$$
\end{theorem}
\begin{proof}
We first prove that case that $x_i \leq x_{n+1} \leq 0.25$:
\begin{lemma}For $D_Y = \text{Uniform}[0,1]$ and $x_{n+1}\leq 0.25$, we have,
$$x^* = \arg \min_{x_i\leq x_{n+1}} \{\mathbbm{E}_{Y}\left[\nkt(R_{n +1}, R_i)\right]\} = 0$$
\end{lemma}
\begin{proof}
In the proving of this lemma, we define $p_i = \mathbbm{P}[y_1\succ_{i} y_2]$ and $p_{n+1} = \mathbbm{P}[y_1\succ_{n+1} y_2]$, and we have,
\begin{equation}\nonumber
\begin{split}
&\frac{\partial \mathbbm{E}[\nkt\left((R_i,R_{n+1})\right)]}{\partial x_i}\\
=&\; \frac{\partial \left(\mathbbm{E}_{y_1,y_2}[p_i(1-p_{n+1})+p_{n+1}(1-p_i)]\right)}{\partial x_i}\\
=&\; \mathbbm{E}\left[(1-2p_{n+1})\frac{\partial p_{i}}{\partial x_i}\right]
\end{split}
\end{equation}
For fixed $y_1$ and $y_2$, we have,
$$\frac{\partial p_i}{\partial x_i} = \frac{e^{-|y_1-x_i|}}{e^{-|y_1-x_i|}+e^{-|y_2-x_i|}}\bigg/\partial x_i = \frac{\sign(y_1-x_i)-\sign(y_2-x_i)}{4\cosh^2\left(\frac{\Delta_{1,2}^{(i)}}{2}\right)}$$
Where $\Delta_{1,2}^{(i)} = |y_2-x_i|-|y_1-x_i|$. By substituting $\frac{\partial p_i}{\partial x_i}$, we have,
\begin{equation}\nonumber
\begin{split}
&\frac{\partial \mathbbm{E}[\nkt\left((R_i,R_{n+1})\right)]}{\partial x_i}\\
=&\;\mathbbm{E}_{y_1,y_2}\left[\frac{e^{-\Delta_{1,2}^{(n+1)}}-1}{e^{-\Delta_{1,2}^{(n+1)}}+1} \cdot \frac{\sign(y_1-x_i)-\sign(y_2-x_i)}{4\cosh^2\left(\frac{\Delta_{1,2}^{(i)}}{2}\right)}\right]\\
=&\;\mathbbm{E}_{y_1,y_2}\,f(y_1,y_2,x_i,x_{n+1})
\end{split}
\end{equation}
Where $\Delta_{1,2}^{(n+1)} = |y_2-x_{n+1}|-|y_1-x_{n+1}|$\\
It is also easy to find that $f(y_1,y_2,x_i,x_{n+1}) = f(y_2,y_1,x_i,x_{n+1})$ and it is safe for us to assume $y_1 < y_2$ for all our following discussions.\\
For $y_2\geq y_1 \geq x_i$ or $x_i\geq y_2\leq y_1$, we always have $\sign(y_1-x_i)-\sign(y_2-x_i) = 0$, thus,
$$\mathbbm{E}_{y_1,y_2}\left[f(y_1,y_2,x_i,x_{n+1})\Big|(y_2\geq y_1 \geq x_i)\vee(x_i\leq y_1 \leq y_2)\right] = 0$$
Then, we discuss $\mathbbm{E}_{y_1,y_2}[f(y_1,y_2,x_i,x_{n+1})\Big|y_1 \leq x_i \leq y_2]$ by the following 3 cases:\\
$\casex$: $y_1\leq x_i$ and $y_2\geq 2x_{n+1}$\\
$\casexx$: $y_1\leq x_i$ and $x_i\leq y_2<2x_{n+1}-x_i$\\
$\casexxx$: $y_1\leq x_i$ and $2x_{n+1}-x_i\leq 2x_{n+1}$\\
\\
We define $g\left(\Delta_{1,2}^{(n+1)}\right) = \frac{e^{-\Delta_{1,2}^{(n+1)}}-1}{e^{-\Delta_{1,2}^{(n+1)}}}$ and we have the following properties of $g\left(\Delta_{1,2}^{(n+1)}\right)$\\
\setlength{\parindent}{1.25em}
\indent $1^{\circ}$ $g\left(\Delta_{1,2}^{(n+1)}\right) = -g\left(-\Delta_{1,2}^{(n+1)}\right)$\\
\indent $2^{\circ}$ $\sign\left[g''\left(\Delta_{1,2}^{(n+1)}\right)\right] = \sign\left[g\left(\Delta_{1,2}^{(n+1)}\right)\right]$ (this shows Concavity and convexity of $g(\cdot)$)\\
\indent $3^{\circ}$ $\Big|g\left(\Delta_{1,2}^{(n+1)}\right)\Big| \leq \frac{1}{2}\Big|\Delta_{1,2}^{(n+1)}\Big|$\\
\setlength{\parindent}{0em}
\\
For $\casex$,
we always have $\Delta_{1,2}^{(i)} \in[2x_{n+1}-2x_i,1-x_i]$, $\Delta_{1,2}^{(n+1)} > 0$ and $\mathbbm{E}\left[\Delta_{1,2}^{(n+1)}\Big|\casex\right] = \frac{1+x_i}{2}-x_{n+1}$. Thus, for this case:
\begin{equation}\nonumber
\begin{split}
&\frac{\partial \left(\mathbbm{E}\left[\nkt(R_i,R_{n+1})\big|\casex\right]\right)}{\partial x_i}\\
=&\; \mathbbm{E}_{y_1,y_2}\left[g\left(\Delta_{1,2}^{(n+1)}\right)\cdot\left.\frac{-2}{4\cosh^2\left(\frac{\Delta_{1,2}^{(i)}}{2}\right)}\right| \casex \right]\\
\geq&\; \mathbbm{E}_{y_1,y_2}\left[g\left(\Delta_{1,2}^{(n+1)}\right)\cdot\left.\frac{-2}{4\cosh^2\left(\frac{1}{2}\right)}\right| \casex \right]\\
\geq&\; \frac{-2}{4\cosh^2\left(\frac{1}{2}\right)}\cdot\\
&\;\mathbbm{E}_{y_1,y_2}\left[\left.\Delta_{1,2}^{(n+1)}g(1)+\left(1-\Delta_{1,2}^{(n+1)}\right)g(0)\right| \casex \right]\\
=&\; \frac{2e(e-1)}{\left(1+e\right)^3}\cdot\left(\frac{1+x_i}{2}-x_{n+1}\right)\\
\end{split}
\end{equation}
For $\casexx$,
we always have $\Delta_{1,2}^{(n+1)} < 0$, $\Delta_{1,2}^{(i)} \in[-x_i,2x_{n+1}-x_i]$ and $\mathbbm{E}\left[\Delta_{1,2}^{(n+1)}\Big|\casexx\right] = -\frac{x_{n+1}}{2}$. Thus, for this case:
\begin{equation}\nonumber
\begin{split}
&\frac{\partial \left(\mathbbm{E}\left[\nkt(R_i,R_{n+1})\big|\casexx\right]\right)}{\partial x_i}\\
=&\; \mathbbm{E}_{y_1,y_2}\left[g\left(\Delta_{1,2}^{(n+1)}\right)\cdot\left.\frac{-2}{4\cosh^2\left(\frac{\Delta_{1,2}^{(i)}}{2}\right)}\right| \casexx \right]\\
\geq&\; \mathbbm{E}_{y_1,y_2}\left[g\left(\Delta_{1,2}^{(n+1)}\right)\cdot\left.\frac{-2}{\left(e^{0}+e^{0}\right)^2}\right| \casexx \right]\\
\geq&\; -\frac{1}{2}\,\mathbbm{E}_{y_1,y_2}\left[\left.\frac{1}{2}\Delta_{1,2}^{(n+1)}\right| \casexx \right]\\
\geq&\; -\frac{x_{n+1}}{8}\\
\end{split}
\end{equation}
For $\casexxx$,
we always have $\Delta_{1,2}^{(i)} \in[x_{n+1}-3x_i,2x_{n+1}]$ and $\mathbbm{E}\left[\Delta_{1,2}^{(n+1)}\Big|\casexxx\right] = 0$.\\
We define $y_1$ and $y_2$'s mirrors to $x_{n+1}$: $y_1'$ and $y_2'$ by $y_2' = 2x_{n+1}-y_1$ and $y_1' = 2x_{n+1}-y_2$. For all $(y_1,y_2)\in \casexxx$, we have, $(y_1',y_2')\in \casexxx$ and $\Delta_{1,2}^{(n+1)} = -\Delta_{1',2'}^{(n+1)}$. Thus, for uniform distributed $Y$, we have,
\begin{equation}\nonumber
\begin{split}
&\frac{\partial \left(\mathbbm{E}\left[\nkt(R_i,R_{n+1})\big|\casexxx\right]\right)}{\partial x_i}\\
=&\; \mathbbm{E}_{y_1,y_2}\left[f(y_1,y_2,x_i,x_{n+1}) + f(y_1',y_2',x_i,x_{n+1}) \left|\right.\right.\\
 &\; \left.\left(\Delta_{1,2}^{(n+1)}>0\right) \land  \left(\casexxx\right) \right]\\
=&\; \mathbbm{E}_{y_1,y_2}\left[g\left(\Delta_{1,2}^{(n+1)}\right)\cdot\left.\left[\frac{-2}{4\cosh^2\left(\frac{\Delta_{1,2}^{(i)}}{2}\right)} - \frac{-2}{4\cosh^2\left(\frac{\Delta_{1',2'}^{(i)}}{2}\right)}\right] \right|\right.\\
 &\; \left.\left(\Delta_{1,2}^{(n+1)}>0\right) \land \left(\casexxx\right) \right]\\
\geq&\; \mathbbm{E}_{y_1,y_2}\left[g\left(\Delta_{1,2}^{(n+1)}\right)\cdot\left.\left[\frac{-2}{4\cosh^2\left(\frac{x_{n+1}}{2}\right)} - \frac{-2}{4\cosh^2(0)}\right] \right|\right.\\
 &\;\left.\left(\Delta_{1,2}^{(n+1)}>0\right) \land \left(\casexxx\right) \right]\\
\geq&\; \left(\frac{-2}{4\cosh^2\left(\frac{x_{n+1}}{2}\right)} - \frac{-2}{4\cosh^2(0)}\right)\times\\
 &\;\mathbbm{E}_{y_1,y_2}\left[\left.-\frac{\Delta_{1,2}^{(n+1)}}{2} \right| \left(\Delta_{1,2}^{(n+1)}>0\right) \land \left(\casexxx\right) \right]\\
\geq&\; \left(\frac{1}{4\cosh^2\left(\frac{x_{n+1}}{2}\right)} - \frac{1}{4\cosh^2(0)}\right)\times\\
 &\;\mathbbm{E}_{y_1,y_2}\left[x_{n+1} \left| \left(\Delta_{1,2}^{(n+1)}>0\right)\right. \land \left(\casexxx\right) \right]\\
=&\; \left(\frac{1}{4\cosh^2\left(\frac{x_{n+1}}{2}\right)} - \frac{1}{4\cosh^2(0)}\right)x_{n+1}\\
\end{split}
\end{equation}
Combining the 3 cases discussed, we have,
\begin{equation}\nonumber
\begin{split}
&\frac{\partial \mathbbm{E}\left[\nkt\left(R_i,R_{n+1}\right)\right]}{\partial x_i}=\frac{\partial \mathbbm{E}\left[\nkt\left(R_i,R_{n+1}\right)\Big| y_1< y_2\right]}{\partial x_i}\\
=\;&\frac{\partial \mathbbm{E}\left[\nkt\left(R_i,R_{n+1}\right)\Big| \casex\right]}{\partial x_i}\cdot\mathbbm{P}[\casex\big|y_1<y_2]+\\
 & \frac{\partial \mathbbm{E}\left[\nkt\left(R_i,R_{n+1}\right)\Big|\casexx\right]}{\partial x_i}\cdot\mathbbm{P}[\casexx\big|y_1<y_2]+\\
&\frac{\partial \mathbbm{E}\left[\nkt\left(R_i,R_{n+1}\right)\Big| \casexxx\right]}{\partial x_i}\cdot\mathbbm{P}[\casexxx\big|y_1<y_2]\\
\geq\;& \frac{2e(e-1)}{\left(1+e\right)^3}\cdot\left(\frac{1+x_i}{2}-x_{n+1}\right)\cdot x_i(1-2x_{n+1})\\
&-\frac{x_{n+1}}{8}x_i(2x_{n+1}-2x_i)+\left(\frac{1}{4\cosh^2\left(\frac{x_{n+1}}{2}\right)} - \frac{1}{4\cosh^2(0)}\right)x_{n+1}x_i^2\\
\geq\;& x_i\left[\frac{2e(e-1)}{\left(1+e\right)^3}\cdot\frac{1}{4}\cdot\frac{1}{2}-\frac{1}{8}\cdot\frac{1}{4}\cdot\frac{1}{2}-0.0155\cdot\frac{1}{4}\cdot\frac{1}{4}\right]\\
\geq\;& 0
\end{split}
\end{equation}
Equal sign is true if and only if $x_i = 0$. And we know that $\mathbbm{E}\left[\nkt\left(R_i,R_{n+1}\right)\right]$ is monotonic increasing in the interval $[0,x_{n+1}]$.
\end{proof}
\setlength{\parindent}{0em}
Using similar technique as Lemma 11.2, we can prove the following lemma for $x_i\geq 1-x_{n+1}$.
\begin{lemma}For $D_Y = \text{Uniform}[0,1]$ and $x_{n+1}\leq 0.25$, we have,
$$x^* = \arg \min_{x_i\geq 1-x_{n+1}} \{\mathbbm{E}_{Y}\left[\nkt(R_{n +1}, R_i)\right]\} = 1-x_{n+1}$$
\end{lemma}

\begin{lemma}For $D_Y = \text{Uniform}[0,1]$, $x_i\in [x_{n+1},\,1-x_{n+1}]$ and $x_{n+1}\leq 0.25$, we have,
$$\mathbbm{E}_{Y}\left[\nkt(R_{n +1}, R_i)\right] \geq \mathbbm{E}_{Y}\left[\nkt(R_{n +1}, R_{n+1'})\right]$$
Where $R_{n+1'}$ is the ranking of $x_{n+1}'$, another agent at the same position as $x_{n+1}$ in latent space.
\end{lemma}
\begin{proof}
We similarly define $p_{n+1'} = \mathbbm{P}[y_1\succ_{n+1'} y_2]$ and it is clear that $p_{n+1'} = p_{n+1}$. Thus, we have,\\
$$\mathbbm{E}_{Y}\left[\nkt(R_{n +1}, R_{n+1}')\right] = \mathbbm{E}_{y_1,y_2}\left[2p_{n+1}(1-p_{n+1})\right]\;\text{and}$$
$$\mathbbm{E}_{Y}\left[\nkt(R_{n +1}, R_i)\right] = \mathbbm{E}_{y_1,y_2}\left[p_{n+1}+(1-2p_{n+1})p_i\right]$$
For any $y_1,y_2 \in [0,x_i+x_{n+1}]$, we define $y_1' = x_i+x_{n+1}-y_1$ and $y_2' = x_i+x_{n+1}-y_2$. It is also clear that $D_Y(y_1)\cdot D_Y(y_2) = D_Y(y_1')\cdot D_Y(y_2')$. If we assume $y_1\geq y_2$, we always have $y_1'<y_2'$. We further define $p_{n+1}' = \mathbbm{P}[y_1'\succ_{n+1} y_2']$ and $p_{i}' = \mathbbm{P}[y_1'\succ_{i} y_2']$. It is clear that $p_{n+1}' = p_i$ and $p_{i}' = p_{n+1}$,and we have,
\begin{equation}\nonumber
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{n+1}')\Big|y_1,y_2\leq x_i+x_{n+1}\right]\\
=\;& \mathbbm{E}_{y_1,y_2}\left[p_{n+1}(1-p_{n+1})+p_i(1-p_i)\Big|x_i+x_{n+1}\geq y_2\geq y_1\right]
\end{split}
\end{equation}
\begin{equation}\nonumber
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{i})\Big|y_1,y_2\leq x_i+x_{n+1}\right]\\
=\;& \mathbbm{E}_{y_1,y_2}\left[p_{n+1}+(1-2p_{n+1})p_i\Big|x_i+x_{n+1}\geq y_2\geq y_1\right]
\end{split}
\end{equation}
Then, we always have,
\begin{equation}\nonumber
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{i})\Big|y_1,y_2\leq x_i+x_{n+1}\right] -\\
& \mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{n+1}')\Big|y_1,y_2\leq x_i+x_{n+1}\right]\\
=\;&\mathbbm{E}_{y_1,y_2}\left[p_{n+1}^2+p_i^2-2p_ip_{n+1}\Big|x_i+x_{n+1}\geq y_2\geq y_1\right]\\
\geq\;& 0\\
\end{split}
\end{equation}
For the case that $y_1\leq x_i+x_{n+1}\leq y_2$ or $y_2\leq x_i+x_{n+1}\leq y_1$, we know that this two subcases are equivalent because of the symmetry of $y_1$ and $y_2$. So, for $y_1\leq x_i+x_{n+1}\leq y_2$, we have,
\begin{equation}\nonumber
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{i})\Big|y_1\leq x_i+x_{n+1}\leq y_2\right] - \\
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{n+1'})\Big|y_1\leq x_i+x_{n+1}\leq y_2\right]\\
=\;&\mathbbm{E}_{y_1,y_2}\left[p_i(1-p_{n+1})+p_{n+1}(1-p_i)-2p_{n+1}(1-p_{n+1})\Big|\right.\\
&\;\;\;\;\;\;\;\;\;\;\;\left.y_1\leq x_i+x_{n+1}\leq y_2\right]\\
=\;&\mathbbm{E}_{y_1,y_2}\left[(p_i-p_{n+1})(1-2p_{n+1})\Big|y_1\leq x_i+x_{n+1}\leq y_2\right]\\
\end{split}
\end{equation}
Because $|y_1-x_{n+1}|\geq|y_2-x_{n+1}|$ for $y_1\leq x_i+x_{n+1}\leq y_2$, $1-2p_{n+1} \leq 0$ is always true. Then,
\begin{equation}\nonumber
\begin{split}
&p_{n+1} = \frac{e^{-|x_{n+1}-y_1|}}{e^{-|x_{n+1}-y_1|}+e^{-|y_2-x_{n+1}|}}\\
=\;&\frac{e^{-\left(|x_{n+1}-y_1|-|x_i-x_{n+1}|\right)}}{e^{-\left(|x_{n+1}-y_1|-|x_i-x_{n+1}|\right)}+e^{-|y_2-x_i|}}\\
\geq\;& \frac{e^{-|x_i-y_1|}}{e^{-|x_i-y_1|}+e^{-|y_2-x_i|}} = p_i
\end{split}
\end{equation}
Thus, we have
\begin{equation}\label{eqn:case1}
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{i})-\nkt(R_{n +1}, R_{n+1'})\Big|\right.\\
&\left.y_1\leq x_i+x_{n+1}\leq y_2\right] \geq 0
\end{split}
\end{equation}
\begin{equation}\label{eqn:case2}
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{i})-\nkt(R_{n +1}, R_{n+1'})\Big|\right.\\
&\left.y_2\leq x_i+x_{n+1}\leq y_1\right] \geq 0
\end{split}
\end{equation}
We also know that
\begin{equation}\label{eqn:case3}
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{i})-\nkt(R_{n +1}, R_{n+1'})\Big|\right.\\
&\left.y_1,y_2\geq x_i+x_{n+1}\right] = 0
\end{split}
\end{equation}
And Lemma 3.4 follows by combining (\ref{eqn:case1}), (\ref{eqn:case2}) and (\ref{eqn:case3}).
\end{proof}
$x_{n+1}\leq 0.25$ part of Theorem 3.1 follows by combining all lemmas above in this section and $x_{n+1}\geq 0.75$ part follows by symmetry of $x_{n+1}\leq 0.25$ part.
\end{proof}










\\
\\
\\
Upper bound for corrected NN algorithm
\begin{theorem}\label{the:CP1}
For $y_1,\cdots, y_m, x_k \in[0,1]$, any $1>\varepsilon>0$ , $x_i = x_j-\varepsilon$, $y_1,\cdots,y_m\sim^{i.i.d.}\mathcal{D}_Y$, $x_k\sim \mathcal{D}_X$ such that $\frac{\max{d_Y}}{\min{d_Y}} = c_Y$ and $\frac{\max{d_X}}{\min{d_X}} = c_X$,  we have,
\begin{equation}\nonumber
\E[D(x_i,x_j)]\geq \frac{ex_i(1-x_i)}{8c_Xc_Y(1+c_Y)(1+e)^2}\varepsilon- O(\varepsilon^2)
\end{equation}
where $d_X$ and $d_Y$ are the probability density function of $D_X$ and $X_Y$ independently.
\end{theorem}
\begin{proof}
We define $p_i = \mathbbm{P}\left[y_1\succ_i y_2\right]$, $p_2 = \mathbbm{P}\left[y_1\succ_j y_2\right]$ and $p_k = \mathbbm{P}\left[y_1\succ_k y_2\right]$. For $x_i\,,\,x_j \in [0,1]$ and $x_j = x_i + \varepsilon$, we have,
\begin{equation}\nonumber
\begin{split}
&\E[D(x_i,x_j)]\\
=\;& \mathbbm{E}_{x_k}\Big|\mathbbm{E}_{y_1,\cdots,y_m,\,R_i,\,R_j,\,R_k}\\
&\;\;\;\;\;\;\;\left[\enkt(R_i,\,R_k)-\enkt(R_j,\,R_k)\right|\Big|\\
=\;& \mathbbm{E}_{x_k}\Big|\mathbbm{E}_{\,y_1,\,y_2,\,R_i,\,R_j,\,R_k}\\
&\;\;\;\;\;\;\;\left\{I\left[(R_i(1)-R_i(2))(R_k(1)-R_k(2))\right] - \right.\\
&\;\;\;\;\;\;\;\; \left.I\left[(R_i(1)-R_i(2))(R_k(1)-R_k(2))\right]\right\}\Big|\\
=\;& \mathbbm{E}_{x_k}\Big|\mathbbm{E}_{\,y_1,\,y_2}\;\left\{\left[p_k(1-p_i)+p_i(1-p_k)\right]-\right.\\
&\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\,\;\;\;\;\;\left.\left[p_k(1-p_j)+p_j(1-p_k)\right]\right\}\Big|\\
=\;& \mathbbm{E}_{x_k}\Big|\mathbbm{E}_{\,y_1,\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\right]\Big|\\
\end{split}
\end{equation}
\\
Then, we derive bound of $(p_i-p_j)(1-2p_k)$ by discussing 3 different cases of $y_1$ and $y_2$:\\
We define Interval $\textcircled{\small{1}} = [0,x_i]$, Interval $\textcircled{\small{2}} = (x_i,x_j)$, and Interval $\textcircled{\small{3}} = [x_j,1]$:\\
\\
\textbf{Case 1: $\bm{y_1,y_2\in\textcircled{\small{1}}}$ or $\bm{y_1,y_2\in\textcircled{\small{3}}}$} \\
\\
\begin{lemma}\label{lem:case1}
for $x_i,x_j,x_k,y_1,y_2\in[0,1]$, $x_j = x_i+\varepsilon$ and $\min\{y_1,y_2\} \geq \max\{x_i,x_j\}$ or $\min\{x_i,x_j\} \geq \max\{y_1,y_2\}$, we have $(p_i - p_j)(1-2p_k) = 0$
\end{lemma}
\begin{proof}
If $y_1,y_2 \geq x_j = x_i+\varepsilon$, we have,
\begin{equation}\nonumber
\begin{split}
p_i =\;& \frac{e^{-(y_1-x_i)}}{e^{-(y_1-x_i)}+e^{-(y_2-x_i)}}\\
=\;& \frac{e^{-(y_1-x_j+\varepsilon)}}{e^{-(y_1-x_j+\varepsilon)}+e^{-(y_2-x_j+\varepsilon)}}\\
=\;& \frac{e^{-(y_1-x_j)}}{e^{-(y_1-x_j)}+e^{-(y_2-x_j)}} = p_j
\end{split}
\end{equation}
And we can similarly get $p_i = p_j$ for the case that $y_1,y_2 \leq x_i = x_j-\varepsilon$\\
Thus, we have, $(p_i - p_j)(1-2p_k) = 0$ considering $-1\leq1-2p_k\leq 1$
\end{proof}

\textbf{Case 2: $\bm{y_1\in\textcircled{\small{1}},\;y_2\in\textcircled{\small{3}}}$ or $\bm{y_1\in\textcircled{\small{3}},\;y_2\in\textcircled{\small{1}}}$} \\
\\
\begin{lemma}\label{lem:case2}
$x_k\in[0,\frac{x_i}{4}],\;y_1\in[0,x_i]$ and $y_2\in[x_j,1]$, we have
\end{lemma}
\begin{equation}\nonumber
\begin{split}
&\bigg|\mathbbm{E}_{\,y_1,\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\right.\\
&\;\;\;\;\;\;\;\;\;\;\;\left.\,\Big|\,x_k\in[0,\frac{x_i}{4}],\;y_1\in[0,x_i],\;y_2\in[x_j,1]\right]\bigg|\\
\geq\;&\frac{ex_i}{2(1+c_Y)(1+e)^2}\varepsilon - O(\varepsilon^2)
\end{split}
\end{equation}
\\
\begin{proof}
we first prove that for all $x_k\in[0,\frac{x_i}{2}],\;y_1\in[0,x_i],\;y_2\in[x_j,1]$, $\left(p_i-p_j\right)(1-2p_k)$ is always negative.\\
It is very clear that $||y_1-x_i|| < ||y_1-x_j||$ and $||y_2-x_i|| > ||y_2-x_j||$. So, we have,
\begin{equation}\nonumber
\begin{split}
&p_i = \frac{e^{-||y_1-x_i||}}{e^{-||y_1-x_i||}+e^{-||y_2-x_i||}}\\
>\;& \frac{e^{-||y_1-x_j||}}{e^{-||y_1-x_j||}+e^{-||y_2-x_i||}}>\frac{e^{-||y_1-x_j||}}{e^{-||y_1-x_j||}+e^{-||y_2-x_j||}} = p_j
\end{split}
\end{equation}
Also, for all $x_k\in[0,\frac{x_i}{2}]$, we have $$\max\limits_{y_1}{||x_k-y_1||} = x_i - x_k\;\;\;\;\text{and}\;\;\;\;\min\limits_{y_2}{||x_k-y_2||} = x_j - x_k = x_i-x_k+\varepsilon$$
Thus, we have $||x_k-y_1|| < ||x_k-y_2||$ and
$$1-2p_k = 1-\frac{2e^{-||y_1-x_k||}}{e^{-||y_1-x_k||}+e^{-||y_2-x_k||}} < 0$$
Thus, we have $(p_i-p_j)(1-2p_k) < 0$ and
\begin{equation}\nonumber
\begin{split}
&\bigg|\mathbbm{E}_{\,y_1,\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\,\Big|\,x_k\in\left[0,\frac{x_i}{4}\right],\;y_1\in[0,x_i],\;y_2\in[x_j,1]\right]\bigg|\\
= \;&\mathbbm{E}_{\,y_1,\,y_2}\left[\left(p_i-p_j\right)(2p_k-1)\,\Big|\,x_k\in\left[0,\frac{x_i}{4}\right],\;y_1\in[0,x_i],\;y_2\in[x_j,1]\right]\\
\geq\;&\mathbbm{E}_{\,y_1,\,y_2}\left[\left(p_i-p_j\right)(2p_k-1)\,\Big|\,x_k\in\left[0,\frac{x_i}{4}\right],\;y_1\in\left[0,\frac{x_i}{2}\right],\;y_2\in[x_j,1]\right]\cdot\mathbbm{P}\left(y_1\in\left[0,\frac{x_i}{2}\right] \,\Big|\, y_1\in\left[0,x_i\right]\right)\\
\geq\;&\frac{1}{1+c_Y}\cdot\mathbbm{E}_{\,y_1,\,y_2}\\
&\left[\left(p_i-p_j\right)(2p_k-1)\,\bigg|\,x_k\in\left[0,\frac{x_i}{4}\right],\;y_1\in\left[0,\frac{x_i}{2}\right],\;y_2\in[x_j,1]\right]\\
\end{split}
\end{equation}
Then, we bound $p_i-p_j$ and $2p_k-1$ on the condition $x_k\in\left[0,\frac{x_i}{2}\right],\;y_1\in\left[0,\frac{x_i}{4}\right],\;y_2\in[x_j,1]$\\
\begin{equation}\nonumber
\begin{split}
&p_j = \frac{e^{-(x_j-y_1)}}{e^{-(x_j-y_1)}+e^{-(y_2-x_j)}}\\
=\;& \frac{e^{-(x_i-y_1)-\varepsilon}}{e^{-(x_i-y_1)-\varepsilon}+e^{-(y_2-x_i)+\varepsilon}}\\
=\;& \frac{e^{-(x_i-y_1)}}{e^{-(x_i-y_1)}+e^{-(y_2-x_i)+2\varepsilon}} \\
=\;& \frac{e^{-(x_i-y_1)}}{e^{-(x_i-y_1)}+e^{-(y_2-x_i)}+2\varepsilon e^{-(y_2-x_i)}}\pm O(\varepsilon^2)\\
=\;& \frac{e^{-(x_i-y_1)}}{e^{-(x_i-y_1)}+e^{-(y_2-x_i)}}\cdot\frac{1}{1+2\varepsilon \frac{e^{-(y_2-x_i)}}{e^{-(x_i-y_1)}+e^{-(y_2-x_i)}}}\\
&\pm O(\varepsilon^2)\\
=\;& p_i\cdot\frac{1}{1+2\varepsilon(1-p_i)}\pm O(\varepsilon^2)\\
=\;& p_i\cdot[1-2\varepsilon(1-p_i)]\pm O(\varepsilon^2)\\
=\;& p_i-2\varepsilon p_i(1-p_i)\pm O(\varepsilon^2)\\
\leq\;& p_i-2\varepsilon \frac{1}{1+e}(1-\frac{1}{1+e})\pm O(\varepsilon^2)\\
\leq\;& p_i- \frac{2e\varepsilon}{(1+e)^2}\pm O(\varepsilon^2)\\
\end{split}
\end{equation}
Thus, it is clear that
$$p_i-p_j\geq \frac{2e\varepsilon}{(1+e)^2}\pm O(\varepsilon^2)$$
For $p_k$, we have,
\begin{equation}\nonumber
\begin{split}
&p_j = \frac{e^{-||x_k-y_1||}}{e^{-||x_k-y_1||}+e^{-||x_k-y_2||}}\\
\geq\;&\frac{e^{-\frac{x_i}{4}}}{e^{-\frac{x_i}{4}}+e^{-\frac{3x_i}{4}}} = \frac{1}{2}\left(1+\frac{x_i}{4}\right)\pm O(\varepsilon^2)
\end{split}
\end{equation}
\emph{Lemma \ref{lem:case2}} follows by combining the bound for $p_i-p_j$ and $2p_k-1$.
\end{proof}

We can get the following lemma for $x_k\in[0,\frac{3+x_j}{4}]$ by symmetry,\\
\\
\begin{lemma}\label{lem:case22}
$x_k\in\left[0,\frac{3+x_j}{4}\right],\;y_1\in[0,x_i]$ and $y_2\in[x_j,1]$, we have
\begin{equation}\nonumber
\begin{split}
&\Bigg|\mathbbm{E}_{\,y_1,\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\,\Big|\right.\\
&\left.\,\,x_k\in\left[0,\frac{3+x_j}{4}\right],\;y_1\in[0,x_i],\;y_2\in[x_j,1]\right]\Bigg|\\
\geq\;&\frac{e(1-x_i)}{2(1+c_Y)(1+e)^2}\varepsilon - O(\varepsilon^2)
\end{split}
\end{equation}
\end{lemma}
It is also clear that Lemma \ref{lem:case2} and Lemma \ref{lem:case22} will still hold if exchange $y_1$ and $y_2$.\\
\\
\textbf{Case 3: $\bm{y_1\in\textcircled{\small{2}}}$ or $\bm{y_2\in\textcircled{\small{2}}}$} \\
\\
\begin{lemma}\label{lem:case3}
If $\exists y\in\{y_1,y_2\}$ $s.t.$ $x_i<y<x_j$, we have
$$\bigg|\mathbbm{E}_{\,y_1,\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\,\Big|\,\left(y_1\in[0,x_i]\right)\vee\left(\;y_2\in[x_j,1]\right)\right]\bigg| = O(\varepsilon)$$
\end{lemma}
\begin{proof}
\begin{equation}\nonumber
\begin{split}
&|p_i-p_j|\\
=\;& \bigg|\frac{e^{-||x_i-y_1||}}{e^{-||x_i-y_1||}+e^{-||y_2-x_i||}}-\frac{e^{-||x_j-y_1||}}{e^{-||x_j-y_1||}+e^{-||y_2-x_j||}}\bigg|\\
\leq\;& \max\\
&\left\{\frac{e^{-||x_j-y_1||+\varepsilon}}{e^{-||x_i-y_1||+\varepsilon}+e^{-||y_2-x_i||-\varepsilon}}-\frac{e^{-||x_j-y_1||}}{e^{-||x_j-y_1||}+e^{-||y_2-x_j||}},\right. \\
&\left.\frac{e^{-||x_i-y_1||-\varepsilon}}{e^{-||x_i-y_1||-\varepsilon}+e^{-||y_2-x_i||+\varepsilon}}-\frac{e^{-||x_j-y_1||}}{e^{-||x_j-y_1||}+e^{-||y_2-x_j||}}\right\}\\
=\;& O(\varepsilon)
\end{split}
\end{equation}
\emph{Lemma \ref{lem:case3}} follows by applying $-1\leq 1-2p_k\leq1$.
\end{proof}

By applying Lemma \ref{lem:case1} - \ref{lem:case3}, for $x_k\in[0,\frac{x_i}{4}]$, we have,
\begin{equation}\nonumber
\begin{split}
&\Big|\mathbbm{E}_{\,y_1,\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\right]\Big|\\
\geq\;&\bigg|\mathbbm{E}_{\,y_1,\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\,\Big|\,\textbf{Case 1}\right]\bigg|\cdot\mathbbm{P}\left(\textbf{Case 1}\right) -\\ &\bigg|\mathbbm{E}_{\,y_1,\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\,\Big|\,\textbf{Case 2}\right]\bigg|\cdot\mathbbm{P}\left(\textbf{Case 2}\right)-\\
&\bigg|\mathbbm{E}_{\,y_1,\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\,\Big|\,\textbf{Case 3}\right]\bigg|\cdot\mathbbm{P}\left(\textbf{Case 3}\right)\\
\geq\;&\frac{ex_i}{2(1+c_Y)(1+e)^2}\varepsilon \cdot \frac{2x_i(1-x_i)}{c_Y} - O(\varepsilon^2) - 0 - O(\varepsilon)\varepsilon\\
=\;&\frac{ex_i^2(1-x_i)}{c_Y(1+c_Y)(1+e)^2}\varepsilon - O(\varepsilon^2)\\
\end{split}
\end{equation}
Similarly, for $x_k\in[0,\frac{3+x_j}{4}]$, we have,
$$\Big|\mathbbm{E}_{\,y_1,\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\right]\Big|\geq\frac{ex_i(1-x_i)^2}{c_Y(1+c_Y)(1+e)^2}\varepsilon - O(\varepsilon^2)$$
Combining $x_k\in\left[0,\frac{3+x_j}{4}\right]$ and $x_k\in\left[0,\frac{x_i}{4}\right]$, we have,
\begin{equation}\nonumber
\begin{split}
&\E[D(x_i,x_j)]\\
=\;& \mathbbm{E}_{x_k}\Big|\mathbbm{E}_{\,y_1,\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\right]\Big|\\
\geq\;& \mathbbm{E}_{x_k}\bigg|\mathbbm{E}_{\,y_1,\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\right]\,\Big|\,x_k\in\left[0,\frac{x_i}{4}\right]\bigg|\\
&\cdot\mathbbm{P}\left(x_k\in\left[0,\frac{x_i}{4}\right]\right)+\\
&\mathbbm{E}_{x_k}\bigg|\mathbbm{E}_{\,y_1,\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\right]\,\Big|\,x_k\in\left[0,\frac{3+x_j}{4}\right]\bigg|\\
&\cdot\mathbbm{P}\left(x_k\in\left[0,\frac{3+x_j}{4}\right]\right)\\
\geq\;& \frac{ex_i^2(1-x_i)}{c_Y(1+c_Y)(1+e)^2}\varepsilon\cdot\frac{x_i}{4c_X}\\
&+\frac{ex_i(1-x_i)^2}{c_Y(1+c_Y)(1+e)^2}\varepsilon\cdot\frac{1-x_i}{4c_X}- O(\varepsilon^2)\\
=\;& \frac{ex_i(1-x_i)}{8c_Xc_Y(1+c_Y)(1+e)^2}\varepsilon- O(\varepsilon^2)\\
\end{split}
\end{equation}
\end{proof}



\begin{proof}
We define $p_i = \mathbbm{P}\left[y_1\succ_i y_2\right]$, $p_2 = \mathbbm{P}\left[y_1\succ_j y_2\right]$ and $p_k = \mathbbm{P}\left[y_1\succ_k y_2\right]$. For $x_i\,,\,x_j \in [0,1]$ and $x_j = x_i + \varepsilon$, we have,
\begin{equation}\nonumber
\begin{split}
&\E[D(x_i,x_j)]\\
=\;& \mathbbm{E}_{x_k}\Big|\mathbbm{E}_{y_1,\cdots,y_m,\,R_i,\,R_j,\,R_k}\\
&\;\;\;\;\;\;\;\left[\enkt(R_i,\,R_k)-\enkt(R_j,\,R_k)\right|\Big|\\
=\;& \mathbbm{E}_{x_k}\Big|\mathbbm{E}_{\,y_1,\,y_2,\,R_i,\,R_j,\,R_k}\\
&\;\;\;\;\;\;\;\left\{I\left[(R_i(1)-R_i(2))(R_k(1)-R_k(2))\right] - \right.\\
&\;\;\;\;\;\;\;\; \left.I\left[(R_i(1)-R_i(2))(R_k(1)-R_k(2))\right]\right\}\Big|\\
=\;& \mathbbm{E}_{x_k}\Big|\mathbbm{E}_{\,y_1,\,y_2}\;\left\{\left[p_k(1-p_i)+p_i(1-p_k)\right]-\right.\\
&\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\,\;\;\;\;\;\left.\left[p_k(1-p_j)+p_j(1-p_k)\right]\right\}\Big|\\
=\;& \mathbbm{E}_{x_k}\Big|\mathbbm{E}_{\,y_1,\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\right]\Big|\\
=\;& \mathbbm{E}_{x_k}\Big|\mathbbm{E}_{\,y_1\leq\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\right]\Big|\\
\end{split}
\end{equation}
The last equal sign comes from symmetry over alternatives. 

To simplify the notation, define the following events: 
\begin{itemize}[noitemsep,topsep=0pt]
\setlength{\itemsep}{0pt}
\setlength{\parskip}{0pt}
\setlength{\parsep}{0pt}
\item $\cale_1$: when $y_1,y_2\in[0,x_i]$ or $y_1,y_2\in[x_j,1]$. 
\item $\cale_2$: when $y_1\in[0,x_i]$ and $y_2\in[x_j,1]$. 
\item $\cale_3$: when $y_1\in[x_i,x_j]$ or $y_2\in[x_i,x_j]$. 
\end{itemize}

Then, we derive bound of $(p_i-p_j)(1-2p_k)$ by discussing 3 different cases of $y_1$ and $y_2$:

\mypara{Case 1. $\mathbbm{E}_{\,y_1\leq\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\mid \cale_1\right]$.}



If $y_1,y_2 \geq x_j = x_i+\varepsilon$, we have,
\begin{equation}\nonumber
\begin{split}
p_i =\;& \frac{e^{-(y_1-x_i)}}{e^{-(y_1-x_i)}+e^{-(y_2-x_i)}}\\
=\;& \frac{e^{-(y_1-x_j+\varepsilon)}}{e^{-(y_1-x_j+\varepsilon)}+e^{-(y_2-x_j+\varepsilon)}}\\
=\;& \frac{e^{-(y_1-x_j)}}{e^{-(y_1-x_j)}+e^{-(y_2-x_j)}} = p_j
\end{split}
\end{equation}
We can similarly get $p_i = p_j$ for $y_1,y_2 \leq x_i$ and we thus have,
$$\mathbbm{E}_{\,y_1\leq\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\mid \cale_1\right] = 0$$

\mypara{Case 2. $\mathbbm{E}_{\,y_1\leq\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\mid \cale_2\right]$.}

we first bound $p_i-p_j$,\\
\begin{equation}\nonumber
\begin{split}
&p_j = \frac{e^{-(x_j-y_1)}}{e^{-(x_j-y_1)}+e^{-(y_2-x_j)}}\\
=\;& \frac{e^{-(x_i-y_1)-\varepsilon}}{e^{-(x_i-y_1)-\varepsilon}+e^{-(y_2-x_i)+\varepsilon}}\\
=\;& \frac{e^{-(x_i-y_1)}}{e^{-(x_i-y_1)}+e^{-(y_2-x_i)+2\varepsilon}} \\
=\;& \frac{e^{-(x_i-y_1)}}{e^{-(x_i-y_1)}+e^{-(y_2-x_i)}+2\varepsilon e^{-(y_2-x_i)}}\pm O(\varepsilon^2)\\
=\;& \frac{e^{-(x_i-y_1)}}{e^{-(x_i-y_1)}+e^{-(y_2-x_i)}}\cdot\frac{1}{1+2\varepsilon \frac{e^{-(y_2-x_i)}}{e^{-(x_i-y_1)}+e^{-(y_2-x_i)}}}\\
&\pm O(\varepsilon^2)\\
=\;& p_i\cdot\frac{1}{1+2\varepsilon(1-p_i)}\pm O(\varepsilon^2)\\
=\;& p_i\cdot[1-2\varepsilon(1-p_i)]\pm O(\varepsilon^2)\\
=\;& p_i-2\varepsilon p_i(1-p_i)\pm O(\varepsilon^2)\\
\geq\;& p_i- \frac{\varepsilon}{2}+ O(\varepsilon^2)\\
\end{split}
\end{equation}
Thus, it is clear that
$$p_i-p_j\leq \frac{\varepsilon}{2}+ O(\varepsilon^2)$$
Because it's always true that $-1\leq 1-2p_k\leq 1$, we have,
$$
\mathbbm{E}_{\,y_1\leq\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\mid \cale_2\right]\leq\frac{\varepsilon}{2}+ O(\varepsilon^2)
$$

\mypara{Case 3. $\mathbbm{E}_{\,y_1\leq\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\mid \cale_3\right]$.}

We first give an upper bound to $|p_i-p_j|$,
\begin{equation}\nonumber
\begin{split}
&|p_i-p_j|\\
=\;& \bigg|\frac{e^{-||x_i-y_1||}}{e^{-||x_i-y_1||}+e^{-||y_2-x_i||}}-\frac{e^{-||x_j-y_1||}}{e^{-||x_j-y_1||}+e^{-||y_2-x_j||}}\bigg|\\
\leq\;& \max\\
&\left\{\frac{e^{-||x_j-y_1||+\varepsilon}}{e^{-||x_i-y_1||+\varepsilon}+e^{-||y_2-x_i||-\varepsilon}}-\frac{e^{-||x_j-y_1||}}{e^{-||x_j-y_1||}+e^{-||y_2-x_j||}},\right. \\
&\left.\frac{e^{-||x_i-y_1||-\varepsilon}}{e^{-||x_i-y_1||-\varepsilon}+e^{-||y_2-x_i||+\varepsilon}}-\frac{e^{-||x_j-y_1||}}{e^{-||x_j-y_1||}+e^{-||y_2-x_j||}}\right\}\\
=\;& O(\varepsilon)
\end{split}
\end{equation}
By applying $-1\leq 1-2p_k\leq1$, we have,
$$\mathbbm{E}_{\,y_1\leq\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\mid \cale_3\right] = O(\varepsilon)$$

By combining all 3 cases discussed above, we have,
\begin{equation}\nonumber
\begin{split}
&\Big|\mathbbm{E}_{\,y_1\leq\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\right]\Big|\\
\leq\;&\sum_{1\leq l\leq 3}\bigg|\mathbbm{E}_{\,y_1\leq\,y_2}\left[\left(p_i-p_j\right)(1-2p_k)\mid \cale_l\right]\bigg|\cdot\mathbbm{P}\left[\cale_l\right]\\
\leq\;&\left(\frac{\varepsilon}{2}+ O(\varepsilon^2)\right)\cdot 2c_Yx_i\cdot c_Y(1-x_j) + O(\varepsilon^2) + 0 + O(\varepsilon)\varepsilon\\
\leq\;&c_Y^2x_i(1-x_i)\varepsilon + O(\varepsilon^2)\\
\end{split}
\end{equation}
By now, we give an universal bound for whatever positions of $x_k$ and Theorem \ref{the:CP1} follows by plugging in $x_k$

\end{proof}



==> old_experienment.tex <==
\section{Experiments}
This section presents the experimental result of corrected nearest-neighbor algorithm and show this algorithm is able to correctly predict the ground-truth probability $\mathbbm{P}\left[y_i\geq_{n+1}y_j\right]$.
\subsection{Synthetic data}
We use synthetic data to show the classical nearest neighbor algorithm works extremely bad for some specific position of $x_{n+1}$. Also, we show the performance of the corrected nearest neighbor algorithm is close to the upper limit of nonparametric approaches

{\color{red} Ao: do I need to mention that m = 6000 is more than enough for predicting NN ?}

In the synthetic dataset, we randomly generated 1200 agents and 6000 alternatives according to $D_X = D_Y = \text{Uniform}[0,5]$. Then we use the three algorithms to predict the ground-truth probability $\mathbbm{P}\left[y_i\geq_{n+1}y_j\right]$. (1) Algorithm \ref{alg:classical}, the classical nearest neighbor algorithm. (2) Algorithm \ref{alg:CNN}, our corrected nearest neighbor algorithm. (3) Algorithm \ref{alg:best}, predicting using the real k-NN of $x_{n+1}$ in latent space. It is noteworthy that Algorithm \ref{alg:best} can't be applied without knowing ground truth because the position of agents in latent space can't be observed directly. It is intuitively true that Algorithm \ref{alg:best} is the upper limit of nearest neighbor algorithm for user-based CF algorithms.

In our experiment, all generated agents were treated as $x_{n+1}$ once, and we show the averaged prediction error for those three algorithms among all positions of $x_{n+1}$ in Figure \ref{fig:CV}.

\begin{figure}
\includegraphics[width = 0.5\textwidth]{CV.PNG}


\caption{Averaged prediction error for classical nearest neighbor and corrected nearest neighbor. Algorithm \ref{alg:classical} got best average prediction error 0.0466, Algorithm \ref{alg:best} for 0.0246 and Algorithm \ref{alg:CNN} for 0.0258.}
\label{fig:CV}

\end{figure}


Then, by fixing $k = 205$, we show how prediction error change with $x_{n+1}$ in Figure \ref{fig:205NN}. It is clear that the error of Algorithm \ref{alg:CNN} is very close to the upper limit of nearest neighbor algorithm for user-based CF algorithms.
\begin{figure}
\includegraphics[width = 0.5\textwidth]{205NN.PNG}
\caption{Prediction error $v.s.$ $x_{n+1}$. Classical nearest neighbor works well when $x_{n+1}$ is positioned at corners or center of $D_Y$. However, the error will be very large for classical nearest neighbor when $x_{n+1}$ is far away from these two places.}
\label{fig:205NN}
\end{figure}

\begin{algorithm}[tb]
   \caption{Upper limit of Nearest-Neighbor}
   \label{alg:best}
\begin{algorithmic}
   \STATE {\bfseries Input:} Agents set $X$, alternatives set $Y$, every agent $x_i$'s real position in latent space
   \FOR{$i=1$ {\bfseries to} $k$ }
   \STATE Find the "real" $i$-th nearest neighbor of $x_{n+1}$ in latent space
   \ENDFOR
   \STATE Use the ranking of those $k$-nearest neighbor to vote for $\mathbbm{P}\left[y_i\geq_{n+1}y_j\right]$.
\end{algorithmic}
\end{algorithm}

\subsection{Real-world data}
{\color{red} Ao: If no real-world data, I can make some figures showing the performance on high-dimensional latent spaces}

==> old_intro.tex <==
\section{Introduction}
Learning preferences of \agents over \alternatives is a fundamental computational learning theory problem. For example, in recommender systems, e-commerce companies estimate users' preferences over unranked \alternatives based on similar \agents' preferences~\cite{Aggarwal:2016:RST:2931100}; product designers estimate the demand curve of a new product based on consumers' past choices~\cite{Berry95:Automobile}; security firms estimate terrorists' preferences based on their past behavior; and political firms estimate campaign options based on voters' preferences~\cite{Liu:2009:LRI}.

In a stylized model, there are $m$ \alternatives and $n + 1$ \agents. We are given \agents' preferences over alternatives, often represented by full rankings over a subset of \alternatives. We are asked to predict the $(n+1)$-th \agent's preferences over pairs of \alternatives that are not specified by the \agent.

This stylized model resembles, from example, the widely studied collaborative filtering problem: we have historical data on $n$ users' rating on $m$ products (e.g., netflix movies). A new user arrives and provides his/her ratings over a subset of items. The collaborative filtering (CF) problem aims to fill in the missing ratings from the new user (here we assume our historical data is a ``full observation'' for exposition purpose).


\subsection{Mystery of nearest neighbor's performance}
Based on how \agents' ratings are processed, CF algorithm are grouped as "numeric setting approaches" and "rank setting approaches":

1. In the numeric setting, \agents' ratings are directly used in those models. We let $M$ be an $m \times n$ matrix so that $M_{i, j}$ is the rating of the $i$-th \agent for \alternative $j$. It could either be a '?' or a numeric value (that's often in $\{1, 2, 3, 4, 5\}$.

2. In the rank setting, \agents' ratings are treated as rankings (with ties). We let $R_i(j)$ the the position of \alternative $\;j$ in the ranking of \agent $\;i$.

\subsubsection{Numeric setting approaches}
Since the early days of the introduction of the collaborative filtering problem, heuristics have been proposed to solve the problem, and have mixed results. In the numeric setting, where users provide only a numeric rating (most often from $\{1,2,3,4,5\}$), one often first \agents mean-square-errors (MSE, or other similar metrics) to measure the similarities between \agents, or between \alternatives:

\mypara{1. MSE between \agents.} Let $M_i$ be the $i$-th row of the matrix. Let $S(i, j)$ be the set of \alternatives that are rated by both \agent $i$ and \agent $j$. We define $\mse(M_i, M_j) = \frac{1}{|S(i, j)|} \sum_{k \in S(i, j)}(M_{i, k} - M_{j, k})^2$.

\mypara{2. MSE between \alternatives.} Let $M^{(i)}$ be the $i$-th column of matrix. Let $T(i, j)$ be the set if users that have rated both $i$ and $j$. We define $\mse(M^{(i)}, M^{(j)}) = \frac{1}{|T(i, j)|} \sum_{ k \in T(i, j)}(M_{k, i} - M_{k, j})^2$.

Then one may use these MSE metrics to measure the closeness between users, or between items. In the past 15 years, researchers have been able to improve the performance of CF algorithm, roughly in the following orders:

\myparab{First generation: memory-based collaborative filtering. }\\ One earliest CF solution is to use MSE between \agents to find \agents "closest" to the new ($n + 1$-th) user. Then based on the intuition that if two users are similar to each other on a subset of items, they they must be similar in other items. So we may use the ratings of the nearest-neighbors of user $n + 1$ to fill in the missing ratings of $n + 1$.

Both positive and negative results were shown to memory-based collaborative filtering. But in general, people observe it is very hard to tune this model. No known large systems still directly use this method.

\myparab{1.5 generation: model-based collaborative filtering.}\\ The model based collaborative filtering assumes a model of the rating, \ie the rating is a hidden function of carefully chosen features. Then, this hidden function were fitted and inferred based on training set.

Model-based collaborative filtering often have improved performance. Careful feature-engineering usually will help to improve the performance. Most recommender system often uses this algorithm as a sub-system.

\myparab{Second generation: item-based collaborative filtering.}
People gradually realize that measuring the similarities between \alternatives instead of between \agents are much more effective. And the item-based collaborative filtering this is one of the most-widely used techniques in production systems.

\subsubsection{Rank setting approaches}
More recent research returns to the non-parametric approach and considers a more robust model. In the more robust model, it is assumed that every \agent gives a partial ranking of them items. The \agent-based nearest-neighbor algorithm then have a natural generalization:

\mypara{Nearest-neighbor based on the Kendall-tau distance.} In this approach, the "distance" between two users is not defined as the MSE of their ratings on the shared set $S(i, j)$. Instead, we look at their rankings, $R_i$ and $R_j$, and use Kendall-tau distance between the two rankings as the distance between users.

\Znote{Q: is MSE or KT distance even a metrics, if users do not rate all the items? A: I'm sure KT is not a metric -- Ao}

It is noteworthy that Rank setting approaches also works for numeric datasets (where users give rating instead of ranking). We can always to convert users' rating into a ranking list with ties. Katz-Samuels \etal showed Nearest-neighbor based on the Kendall-tau distance algorithm work well for noise-less data. Tie-yan liu has some papers justifying the efficacy of the KT-distance based approach, with some empirical justification {\color{red} Didn't find Tieyan Liu's paper on this topic, need help from Zhenming}. Even though this algorithm is theoretically elegant and backed up by some experiments, it seems KT distance based non-parametric algorithm is not effective in practice.

{\color{red} Terminology: numeric-based vs non-parametric?}

\Znote{This paper could be relevant: Item-Based Collaborative Filtering Recommendation}

{\color{red} Ao: This part need further polish / make it more organized, but I'm not sure how to do it.}\\
\myparab{Discrepancies between theory and practice.}
Below are the major contradictions/discrepancies between academic research and practical systems:

\mypara{1. Item-based CF is better than user-based CF.} Item-based approach has been known to be much more efficient than user-based approach, across a wide range of datasets ({\color{red} will we be able to find citations?}) While there are explanation on this discrepancy, they do not seem to be convincing.

\mypara{2. Non-parametric approach never used in practical systems.} Despite recent works have justified the efficacy of the non-parametric approach, they rarely perform well in practice. In other words, the theoretical analysis seems inconsistent with empirical observations.

\mypara{3. Non-parametric approach cannot beat model based approach, even for large datasets.} Non-parametric approaches have been known to be more flexible/powerful models. The drawback is that larger datasets are needed. But in practice, even with the presence of very large datasets, we are unable to observe prediction improvement.
{\color{red} 2 and 3 are closely related. We may need to consolidate.}


\subsection{Our contributions}
We introduce a simple, non-parametric model by naturally generalizing Plackett-Luce model, to explain all of the above performance discrepancies:

\mypara{n1. Incorrectness of the nearest-neighbor.} Under our model, the algorithm that uses nearest neighbors using Kendall-tau distance is \emph{provably incorrect.} This shall be contrasted to Katz-Samuels \etal, where nearest-neighbor algorithm is provably correct for noise-less data. A key difference between their model and our model is that they assume deterministic utility function (this corresponds to making assumption that the observed data is ``noiseless'') while we assume a random utility model. In most machine learning algorithm, an algorithm that works for noiseless setting often also work for the noisy setting. But this is not the case in our setting. By introducing a small amount of noises, we see that the structure of the problem got significantly altered.

\mypara{n2. Incorrectness of the MSE for user-based algorithm.} Our technique can be further generated to show that MSE-based approach to find nearest neighbors (in the numeric setting) also will provably give biased results.
\Znote{I think it is possible to generalize the results?}

Then we move to the positive results.

\mypara{p1. A corrected user-based algorithm.} We define a new metrics to measure the similarities between \agents. Then we show that when we use nearest-neighbor algorithm on the new metrics, our estimator converges at large samples, and it requires only polynomial amount of data. {\color{red} Ao: I think we may need to avoid the word "metric" because we can't prove our "measure" is a metric.}\\

\mypara{p2. Generalizing the new techniques to item-based algorithm.} We can rely on the same intuition to generalize our algorithm to develop nearest neighbor algorithm based on item similarities.

\mypara{p3. Item-based algorithm is equivalent to ours.} Finally, we show that that the item-based algorithm (that uses rating, rather than ranking data) is in fact a natural generalization of our algorithm.



{\color{blue} We complement our results by extensively evaluate
xxxxx datasets.}


{\color{blue} ZL's notes:
We need to be able to discuss: an alternative way of explaining why item-based collaborative filtering is better than user-based collaborative filtering: there are fewer items than users. Thus, item-based comparison is more reliable. How can we verify that whether the effectiveness of item-based algorithm is because of the sample complexity (the explanation above), or because of random utility model.

ZL: If effect comes from the random utility model, then we will have a small subset of users that are being closest to a large portion of people. But if the effect comes from noisy observation. Then we will not be able to see such a subset.}

==> old_lower.tex <==
\section{Old lower bound}

Then, we prove the minimum of $\E[D(x_i,x_j)]$ outside the $x_i$'s neighborhood is none-zero.

Then, we prove that for any $x_i$ out of $x_j$'s neighborhood, we have $\E[D(x_i,x_j)] > 0$.
\begin{theorem}\label{the:CP2}
For $y_1,\cdots, y_m, x_1,\cdots,x_{n+1} \in[0,1]$, any $1>\varepsilon>0$ , $|x_i - x_j|\geq\varepsilon$, $y_1,\cdots,y_m\sim^{i.i.d.}\mathcal{D}_Y$, $x_k\sim \mathcal{D}_X$ such that $\frac{\max{d_Y}}{\min{d_Y}} = c_Y$ and $\frac{\max{d_X}}{\min{d_X}} = c_X$,  we have,
\begin{equation}\nonumber
\E[D(x_i,x_j)] > 0
\end{equation}
\end{theorem}
\begin{proof}
We first define a similar as we used in the proof of Theorem \ref{thm:wrong} : $\calf_0(x) \equiv  \E_Y[\nkt(R_{k}, R_x) \mid x_k = 0]$. Similar to the calculation of $d\calf(x)/dx$, we have,
$$\frac{d\calf_0(x)}{dx} = \E_{y_1, y_2}\left[(1-2p_0)\frac{dp}{dx}\right].$$
where $p_0 = \mathbbm{P}[y_1\succ_{k}y_2 \mid x = 0 ]$
Let $\deltaz = y_2 - y_1$ and $\deltax = |y_2 - x| - |y_1 - x|$. We have
\begin{eqnarray*}
& & \E_{y_1, y_2}\left[(1-2p_0)\frac{dp}{dx}\right]\\
& = & \E_{y_1, y_2}\left[\frac{e^{-\deltaz} - 1}{e^{-\deltaz} + 1}\cdot \frac{\sign(y_1 - x) - \sign(y_2 - x)}{4\cosh^2(\deltax/2) }\right] \\
& = & \E_{y_1 < y_2}\left[\frac{e^{-\deltaz} - 1}{e^{-\deltaz} + 1}\cdot \frac{\sign(y_1 - x) - \sign(y_2 - x)}{4\cosh^2(\deltax/2) }\right]
\end{eqnarray*}
The last equation holds because $y_1$ and $y_2$ are symmetric. To simplify the notation, let $\Phi_0(y_1, y_2, x_i) = \frac{e^{-\deltaz} - 1}{e^{-\deltaz} + 1}\cdot \frac{\sign(y_1 - x) - \sign(y_2 - )}{4\cosh^2(\deltax/2) }$ (sometimes we simply use $\Phi_0$ when the context is clear).

Then, we discuss the value of $\frac{d\calf(x)}{dx}$ by the following two cases:

Case 1: $y_1,y_2\geq x$ or $y_1,y_2\leq x$\\
It is easy to check that we always have $\sign(y_1 - x) - \sign(y_2 - x) = 0$ for this case. Thus, we have $$\E[\Phi_0 \mid \text{Case 1}] = 0$$

Case 2: $y_2\geq x\geq y_1$\\
It is easy to check that we always have $\sign(y_1 - x) - \sign(y_2 - x) = -2$ for this case. Also, considering $\deltaz > 0$, we know $\Phi_0 > 0$ for Case 2. By defining Case 2.1 as
$y_1\leq\frac{x}{2}\;\land\; y_2\geq\frac{1+x}{2}$, we have,
\begin{eqnarray*}
& & \E_{y_1\leq y_2}[\Phi_0 \mid \text{Case 2}]\\
& \geq & \E_{y_1 \leq y_2}\left[\Phi_0 \mid \text{Case 2.1}\right]\cdot\; \mathbbm{P}\left[\text{Case 2.1}\mid \text{Case 2}\right]\\
\end{eqnarray*}
For Case 2.1, we have $\deltaz > \frac{1}{2}$, $\deltax < 1$  and we have,
\begin{eqnarray*}
& & \E_{y_1\leq y_2}[\Phi_0 \mid \text{Case 2.1}]\\
& = & \E_{y_1 \leq y_2}\left[\frac{e^{-\deltaz} - 1}{e^{-\deltaz} + 1}\cdot \frac{-2}{4\cosh^2(\deltax/2) }\mid \text{Case 2.1}\right] \\
& \geq & \E_{y_1 \leq y_2}\left[\frac{e^{-0.5} - 1}{e^{-0.5} + 1}\cdot \frac{-2}{4\cosh^2(0.5) }\mid \text{Case 2.1}\right] \\
& \gtrsim &0.0963 
\end{eqnarray*}
Combining the two cases above, we have,
 \begin{eqnarray*}
& & \frac{d\calf_0(x)}{dx} = \E_{y_1\leq y_2}[\Phi_0]\\
& \geq & \E_{y_1 \leq y_2}\left[\Phi_0 \mid \text{Case 2.1}\right]\cdot\; \mathbbm{P}\left[\text{Case 2.1}\right]\\
& \geq & 0.0963\times2\left(\frac{x}{2}\cdot\frac{1}{1+c_Y}\right)\left(\frac{1-x}{2}\cdot\frac{1}{1+c_Y}\right)\\
& = & \frac{0.0963}{2\left(1+c_Y\right)^2}\;x(1-x)\\
\end{eqnarray*}
We further bound $\left|\calf_0(x_{i}) - \calf_0(x_{j})\right|$ by integral, it is safe to assume $x_j \geq x_i$ and the case of $x_j < x_i$ follows by symmetry.
 \begin{eqnarray*}
& &\left| \calf_0(x_{i}) - \calf_0(x_{j})\right|\\
& = & \left|\int_{x_i}^{x_j}\frac{d\calf_0(x)}{dx} dx\right|\\
& \geq & \frac{0.0963}{2\left(1+c_Y\right)^2}\;\left|\frac{1}{2}(x_j^2-x_i^2)-\frac{1}{3}(x_j^3-x_i^3)\right|\\
& = & \frac{0.0963(x_j-x_i)}{12\left(1+c_Y\right)^2}\;\left|3x_j(1-x_j)+3x_i(1-x_i)+(x_i+x_j)^2\right|\\
\end{eqnarray*}
We similarly define $\calf_1(x) \equiv  \E_Y[\nkt(R_{k}, R_x) \mid x_k = 1]$. By symmetry, we have,
 \begin{eqnarray*}
& &\left| \calf_1(x_{i}) - \calf_1(x_{j})\right|\\
& \geq & \frac{0.0963(x_j-x_i)}{12\left(1+c_Y\right)^2}\cdot\\
& &  \left|3x_j(1-x_j)+3x_i(1-x_i)+(2-x_i-x_j)^2\right|\\
\end{eqnarray*}
It is also easy to show that $\left.\frac{d\calf(x)}{dx}\right|_{x=0} = \left.\frac{d\calf(x)}{dx}\right|_{x=1} = 0$ for arbitrary positions of $x_{n+1}$. By selecting $x_k$ within interval $[0,\delta]$, we have,
 \begin{eqnarray*}
& &\E[D(x_i,x_j)]\\
& = & \E_X\left|\E_Y[\nkt(R_i, R_k)]-\E_Y[\nkt(R_j, R_k)]\right|\\
& = & \E_X\left[\left|\E_Y[F_{ik}]-\E_Y[F_{jk}]\right|\mid x_k\in [0,\delta]\right]\cdot\\
& & \mathbbm{P}[x_k\in [0,\delta]]+\\
& & \E_X\left[\left|\E_Y[F_{ik}]-\E_Y[F_{jk}]\right|\mid x_k\in [1-\delta,1]\right]\cdot\\
& & \mathbbm{P}[x_k\in [1-\delta,1]]\\
& \geq & \frac{\delta}{1+C_X}\left[\left|\calf_0(x_{i}) - \calf_0(x_{j})\right|-O(\delta^2)\right]+\\
&  & \frac{\delta}{1+C_X}\left[\left|\calf_1(x_{i}) - \calf_1(x_{j})\right|-O(\delta^2)\right]\\
& \geq & \frac{\delta}{1+C_X}\cdot\frac{0.0963(x_j-x_i)}{48\left(1+c_Y\right)^2}-O(\delta^2)\\
& > & 0
\end{eqnarray*}


\end{proof}
{\color{blue}Zhenming: hello
\begin{eqnarray*}
& & \|\E_Y[\nkt(R_i, R_k)]-\E_Y[\nkt(R_j, R_k)]\| \mid x_{k} \in [0, \delta] \\
& & = \left|\calf_0(x_{i}) - \calf_0(x_{j})\right|-O(\delta^2).
\end{eqnarray*}

\begin{eqnarray*}
& & \left|\E_Y[\nkt(R_i, R_k)]-\E_Y[\nkt(R_j, R_k)]\right| \\
& = & |\calf_{x_k}(x_i) - \calf_{x_k}(x_j)|
\end{eqnarray*}
\begin{eqnarray*}
& &  |\calf_{x_k}(x_i) - \calf_{x_k}(x_j)| \mid x_k \in [0,\delta] \\
& = &  \left|\calf_0(x_{i}) - \calf_0(x_{j})\right|-O(\delta^2).
\end{eqnarray*}

$$|\calf_{x_k}(x_i) - \calf_0(x_i)|.$$
$$\calf(x) \equiv  \E_Y[\nkt(R_{n+1}, R_x)]$$
}

Theorem \ref{the:CP1} and Theorem \ref{the:CP2} together show that $x^* = x_{n+1}$ is the only global minimum of $\E[D(x_{n+1},x)]$ by applying the continuity of $\E[D(x_{n+1},x)]$. We also know from the tail bound that $D(x_{n+1},x)$ converge with exponential rate $\E[D(x_{n+1},x)]$ on the condition that $n = \text{Polynomial}(m)$. All result in this section sums up to the conclusion that Algorithm \ref{alg:CNN} (corrected nearest neighbor) will find the nearest neighbor when $m$ is large.


==> old_tail.tex <==
\section{Old tail bounds}
\begin{definition} [Estimator for partial rankings] For $x_i$ gives full rankings on $O_i$, $x_j$ gives full rankings on $O_j$,
\begin{equation}\label{eqn:enkt}
\begin{split}
\enkt(R_i, R_j)=  &\;  \frac{1}{\left\lfloor \frac { m_{ij}} {2}\right\rfloor} \sum_{k = 1}^{\left\lfloor \frac { m_{ij}} {2}\right\rfloor} I\left[\left(R_i(y_{2k-1}^{(ij)}) - R_i(y_{2k}^{(ij)})\right)\right.\\
 &\left.\cdot\left(R_j(y_{2k - 1}^{(ij)}) - R_j(y_{2k}^{(ij)}) \right)\right]\\
\end{split}
\end{equation}
where $m_{ij}$ is the number of alternatives $x_i$ and $x_j$ both ranked, and $y_{k}^{(ij)}$ is the $k^{th}$ ranked both by $x_i$ and $x_j$.
\end{definition}


{\color{green} ZL: most of them needs to be moved out. 
\section{A corrected nearest-neighbor algorithm}
This section presents a new nearest-neighbor based algorithm that is guaranteed to converge to the ground-truth at polynomial rate (\ie only a polynomial number of samples is needed). Then we will generalize the result to the case where we don't have full observation.

\myparab{Plug-in estimator.} The above nearest neighbor procedure relies on the knowledge of the normalized Kendall-tau distance between two agents, which cannot be observed. Here, we can simply plug in an arbitrary normalized Kendall-tau estimator. We use the following estimator:

Here, our goal is to estimate $\E[\nkt(R_i, R_j)\,\big|\,x_i, x_j]$. We group $y_i$'s as pairs so that the $i$-th pair consists of $\{y_{2i - 1},y_{2i}\}$. Note that the pairs are independent. Our estimator is
\begin{definition} [Estimator for partial rankings] For $x_i$ gives full rankings on $O_i$, $x_j$ gives full rankings on $O_j$,
\begin{equation}\label{eqn:enkt}
\begin{split}
\enkt(R_i, R_j)=  &\;  \frac{1}{\left\lfloor \frac { m_{ij}} {2}\right\rfloor} \sum_{k = 1}^{\left\lfloor \frac { m_{ij}} {2}\right\rfloor} I\left[\left(R_i(y_{2k-1}^{(ij)}) - R_i(y_{2k}^{(ij)})\right)\right.\\
 &\left.\cdot\left(R_j(y_{2k - 1}^{(ij)}) - R_j(y_{2k}^{(ij)}) \right)\right]\\
\end{split}
\end{equation}
where $m_{ij}$ is the number of alternatives $x_i$ and $x_j$ both ranked, and $y_{k}^{(ij)}$ is the $k^{th}$ ranked both by $x_i$ and $x_j$.
\end{definition}
Intuitively, the probability that the signs that $R_i(y_{2k-1}) - R_i(y_{2k})$ and $R_j(y_{2k - 1}) - R_j(y_{2k})$ are inconsistent is proportional to the Kendall-tau distance conditioned on $x_i$ and $x_{j}$. By summing up independent terms,
$$I\left[(R_i(y_{2k-1}^{(ij)}) - R_i(y_{2k}^{(ij)}))(R_j(y_{2k - 1}^{(ij)}) - R_j(y_{2k}^{(ij)}) )\right]$$
after appropriate scaling, we can obtain an accurate estimate of $\E[\nkt(R_i, R_j)|x_i, x_j]$.


\myparab{Features based on all-pair normalized Kendall-tau distance.} We associate each agent $i \in [n + 1]$ with a feature $F_i \in R^{n}$ so that $F_{i, j}$ is $\enkt(R_i, R_j)$. The distance function between agent $i$ and agent $j$ is defined as
\begin{equation}
D(x_i, x_j) = \frac{1}{\left|O_i^{(j)}\right|-2}\sum_{x_k\in O_i^{(j)}\setminus \{x_i, x_j\}}|F_{i, k} - F_{j, k}|.
\end{equation}
{\color{red} Q: might be change $x_k \in O_i^{(j)}\setminus \{x_i, x_j\}$ to $k \in [n+1]\setminus \{i, j\}$?}
Our nearest-neighbor algorithm (Algorithm \ref{alg:CNN}) on input $R_{n + 1}$ will return the $k$-nearest neighbors of $R_{n + 1}$ under the metrics $D(\cdot, \cdot)$.
\begin{algorithm}[tb]
   \caption{Corrected Nearest-Neighbor Algorithms}
\begin{algorithmic}
   \STATE {\bfseries Input:} Agents set $X$, Alternative set $Y$, every agent $x_i$'s ranking over $O_i\subseteq Y$
   \FOR{$i=1$ {\bfseries to} $n+1$ }
   \STATE Compute $O_{n+1}^{(i)} = O_{n+ 1} \cap O_i$
   \ENDFOR
   \STATE Find $i^* = \arg \min_{i \in [n]} \left\{D(x_i, x_{n+1})\right\}$
   \STATE Use $R_{i^*}$ to reconstruct the full ranking $\hat R_{n + 1}$.
\end{algorithmic}
\end{algorithm}

\subsection{Tail bound for distance functions}
In this section, we bound the tail probability that $D(x_i, x_j)$ is far away from $\E[D(x_i, x_j)]$ for the setting that all agents give rankings on $\frac{m}{c}$ alternatives randomly chosen from $Y$.

\begin{theorem}
For $x_{1},\cdots,x_{n+1}\in[0,1]^d$, $y_1,\cdots,y_m\in[0,1]^d$, and every agent randomly rank $\frac{m}{c}$ alternatives, we have,
$$\mathbbm{P}\left[\left|D(x_i,x_j)-\mathbbm{E}\left[D(x_i,x_j)\right]\right| \geq \delta\right] \leq 4n\left(1-\frac{1}{c}+\frac{1}{ce^\alpha}\right)^{\frac{m}{c}}$$
where $\alpha = \frac{\delta^2}{24}\cdot\frac{2e^{\sqrt{d}}}{\left(1+e^{\sqrt{d}}\right)^2}>0$
\end{theorem}
\begin{proof}
We first give a lower bound on $\mathbbm{E}\left[\enkt(R_i,R_j)\right]$.

\begin{lemma}
Letting $x_1,x_2\in[0,c_D]^d$ and $y_1,\cdots,y_m\in[0,c_D]^d$, for $R_1$ and $R_2$, two rankings generated by $x$ and $y_1,\cdots,y_m$ through randomized setting, we have,
$$\mathbbm{E}[\enkt(R_1,R_2)] \geq \frac{2e^{\left(c_D\sqrt{d}\right)}}{\left[1+e^{\left(c_D\sqrt{d}\right)}\right]^2}$$
\end{lemma}
\begin{proof}
We define $p_1^{(i,j)} = \mathbbm{P}\left[y_i\succ_{1}y_j\right]$ and $p_2^{(i,j)} = \mathbbm{P}\left[y_i\succ_{2}y_j\right]$. For both $p_1^{(i,j)}$ and $p_2^{(i,j)}$ we have,
\begin{equation}\nonumber
\begin{split}
&p_1^{(i,j)},\;p_2^{(i,j)} \leq \max\left\{\frac{e^{-||y_i-x_1||}}{e^{-||y_i-x_1||}+e^{-||y_j-x_1||}}\right\}\\
\leq \;&\frac{1}{e^{-c_D\sqrt{d}}+1} = p_{\max}
\end{split}
\end{equation}
\begin{equation}\nonumber
\begin{split}
&p_1^{(i,j)},\;p_2^{(i,j)} \geq \min\left\{\frac{e^{-||y_i-x_1||}}{e^{-||y_i-x_1||}+e^{-||y_j-x_1||}}\right\}\\
\geq \;& \frac{e^{-c_D\sqrt{d}}}{e^{-c_D\sqrt{d}}+1} = p_{\min}
\end{split}
\end{equation}
For normalized Kendall-tau distance, we have,
\begin{equation}\nonumber
\begin{split}
&\;\;\;\;\;\mathbbm{E}[\nkt(R_1,R_2)]\\
&= \frac{1}{\binom{m}{2}}\sum\limits_{i\not=j}\mathbbm{E}\left[I\left([R_1(i)-R_1(j)][R_2(i)-R_2(j)]\right)\right]\\
&= \frac{1}{\binom{m}{2}}\sum\limits_{i\not=j}\left[p_1^{(i,j)}\left(1-p_2^{(i,j)}\right)+p_2^{(i,j)}\left(1-p_1^{(i,j)}\right)\right]\\
&= \frac{1}{\binom{m}{2}}\sum\limits_{i\not=j}\left[p_1^{(i,j)}+p_2^{(i,j)}-2p_1^{(i,j)}p_2^{(i,j)}\right]\\
&\geq \frac{1}{\binom{m}{2}}\sum\limits_{i\not=j}\min\left\{2p_{\max}-2p_{\max}^2,\,2p_{\min}-2p_{\min}^2\right\}\\
&= \frac{1}{\binom{m}{2}}\sum\limits_{i\not=j}2\cdot\frac{1}{e^{-c_D\sqrt{d}}+1}\cdot\frac{e^{-c_D\sqrt{d}}}{e^{-c_D\sqrt{d}}+1}\\
&= \frac{2e^{\left(c_D\sqrt{d}\right)}}{\left[1+e^{\left(c_D\sqrt{d}\right)}\right]^2}
\end{split}
\end{equation}
Similarly, for $x_1,x_2,y_1,\cdots,y_m\in A$ $s.t.$ $\sup\limits_{a,b\in A}||a-b|| = D$, we have,
$$\mathbbm{E}[\nkt(R_1,R_2)]\geq \frac{2e^D}{\left(1+e^D\right)^2}$$
\end{proof}


Then, we use Chernoff bound to bound the tail probability of $\enkt$, we use $X_k^{(ij)}$ to denote the random variable $I\left[(R_i(y_{2k-1}^{(ij)}) - R_i(y_{2k}^{(ij)}))(R_j(y_{2k - 1}^{(ij)}) - R_j(y_{2k}^{(ij)}) )\right]$ in this section. And it is very clear that $X_1^{(ij)},\cdots,X_{m_{ij}}^{(ij)}$ are $i.i.d.$ (do not fix $y_i$s here).

\begin{equation}\nonumber
\begin{split}
&\mathbbm{P}\left[\big|\enkt(R_i,R_j)-\mathbbm{E}\left[\enkt(R_i,R_j)\right]\big|\right.\\
&\;\;\;\;\left. \geq \delta\,\mathbbm{E}\left[\enkt(R_i,R_j)\right] \right]\\
=\;& \mathbbm{P}\left[\left|\frac{2}{m_{ij}}\sum_{k=1}^{m_{ij}/2}X_k^{(ij)}-\mathbbm{E}\left[X_k^{(ij)}\right]\right| \geq \delta\,\mathbbm{E}\left[X_k^{(ij)}\right] \right]\\
=\;& \mathbbm{P}\left[\left|\sum_{k=1}^{m_{ij}/2}X_k^{(ij)}-\frac{m_{ij}}{2}\mathbbm{E}\left[X_k^{(ij)}\right]\right| \geq \delta\,\frac{m_{ij}}{2}\mathbbm{E}\left[X_k^{(ij)}\right] \right]\\
\leq\;& 2\exp\left(-\,\frac{\delta^2\, m_{ij}}{6}\mathbbm{E}\left[X_k^{(ij)}\right]\right)\\
=\;& 2\exp\left(-\,\frac{\delta^2\, m_{ij}}{6}\mathbbm{E}\left[\enkt(R_i,R_j)\right]\right)\\
\leq\;& 2\exp\left(-\,\frac{\delta^2\, m_{ij}}{6}\cdot\frac{2e^{\sqrt{d}}}{\left(1+e^{\sqrt{d}}\right)^2}\right)\\
\end{split}
\end{equation}
where $m_{ij}$ denote the number of alternatives ranked by both $x_i$ and $x_j$, we also have $m_{ij}$ follows hypergeometric distribution such that,\\
$$\mathbbm{P}[m_{ij} = l] = \frac{\binom{\frac{m}{c}}{l}\binom{m-\frac{m}{c}}{\frac{m}{c}-l}}{\binom{m}{\frac{m}{c}}}$$
Letting $Y_{i,n+1}^{(k)} = \enkt(R_i,R_k)-\enkt(R_{n+1},R_k)$, we have,
\begin{equation}\nonumber
\begin{split}
&\mathbbm{P}\left[\left|Y_{i,n+1}^{(k)}-\mathbbm{E}\left[Y_{i,n+1}^{(k)}\right]\right| \geq \delta\,\bigg|\,m_{ik}=l_1,\;m_{k(n+1)}=l_2\right]\\
\leq\;& \mathbbm{P}\left[\left(\big|\enkt(R_i,R_k)-\mathbbm{E}\left[\enkt(R_i,R_k)\right]\big| \geq \frac{\delta}{2}\right)\bigcup\right.\\
&\;\;\left(\big|\enkt(R_{n+1},R_k)-\mathbbm{E}\left[\enkt(R_{n+1},R_k)\right]\big| \geq \frac{\delta}{2}\right)\\
&\;\;\left.\bigg|\,m_{ik}=l_1,\;m_{k(n+1)}=l_2\right]\\
\leq\;& \mathbbm{P}\left[\big|\enkt(R_i,R_k)-\mathbbm{E}\left[\enkt(R_i,R_k)\right]\big| \geq \frac{\delta}{2}\right.\\
&\;\;\;\;\left.\bigg|\,m_{ik}=l_1\right]+\\
&\mathbbm{P}\left[\big|\enkt(R_{n+1},R_k)-\mathbbm{E}\left[\enkt(R_{n+1},R_k)\right]\big| \geq \frac{\delta}{2}\,\right.\\
&\;\;\;\;\left.\bigg|m_{k(n+1)}=l_2\right]\\
\leq\;& 2\exp\left(-\,\frac{\delta^2\, l_1}{24}\cdot\frac{2e^{\sqrt{d}}}{\left(1+e^{\sqrt{d}}\right)^2}\right) +\\
& 2\exp\left(-\,\frac{\delta^2\,l_2}{24c_1}\cdot\frac{2e^{\sqrt{d}}}{\left(1+e^{\sqrt{d}}\right)^2}\right)\\
=\;& 2e^{-\alpha l_1} + 2e^{-\alpha l_2}\;\;\;\;\left(\alpha = \frac{\delta^2}{24}\cdot\frac{2e^{\sqrt{d}}}{\left(1+e^{\sqrt{d}}\right)^2}>0\right)\\
\end{split}
\end{equation}
Thus,
\begin{equation}\nonumber
\begin{split}
&\mathbbm{P}\left[\left|Y_{i,n+1}^{(k)}-\mathbbm{E}\left[Y_{i,n+1}^{(k)}\right]\right| \geq \delta\right]\\
=\;&\sum_{l_1=0}^{m/c}\sum_{l_2=0}^{m/c}\mathbbm{P}\left[\left|Y_{i,n+1}^{(k)}-\mathbbm{E}\left[Y_{i,n+1}^{(k)}\right]\right| \geq \delta\right.\\
&\left.\bigg|\,m_{ik}=l_1,\;m_{k(n+1)}=l_2\right] \cdot\mathbbm{P}\left[m_{ik}=l_1,\;m_{k(n+1)}=l_2\right]\\
\leq\;&\sum_{l_1=0}^{m/c}\sum_{l_2=0}^{m/c}(2e^{-\alpha l_2}+2e^{-\alpha l_1}) \cdot\left[\frac{\binom{\frac{m}{c}}{l_1}\binom{m-\frac{m}{c}}{\frac{m}{c}-l_1}}{\binom{m}{\frac{m}{c}}} \cdot \frac{\binom{\frac{m}{c}}{l_2}\binom{m-\frac{m}{c}}{\frac{m}{c}-l_2}}{\binom{m}{\frac{m}{c}}}\right]\\
=\;& \sum_{l_1=0}^{m/c} 2e^{-\alpha l_1}\frac{\binom{\frac{m}{c}}{l_1}\binom{m-\frac{m}{c}}{\frac{m}{c}-l_1}}{\binom{m}{\frac{m}{c}}} + \sum_{l_2=0}^m 2e^{-\alpha l_2}\frac{\binom{\frac{m}{c}}{l_2}\binom{m-\frac{m}{c}}{\frac{m}{c}-l_2}}{\binom{m}{\frac{m}{c}}}\\
\leq\;& 4\left(1-\frac{1}{c}+\frac{1}{ce^\alpha}\right)^{\frac{m}{c}}\\
\end{split}
\end{equation}
The last "$\leq$" sign comes from supplementary Lemma 1.\\
For the distance function $D(x_i,x_j)$, we have,
\begin{equation}\nonumber
\begin{split}
&\mathbbm{P}\left[\left|D(x_i,x_j)-\mathbbm{E}\left[D(x_i,x_j)\right]\right| \geq \delta\right]\\
\leq\;& \sum_{k\not\in\{i,n+1\}}\mathbbm{P}\left[\left|Y_{i,n+1}^{(k)}-\mathbbm{E}\left[Y_{i,n+1}^{(k)}\right]\right| \geq \delta\right]\\
\leq\;& 4n\left(1-\frac{1}{c}+\frac{1}{ce^\alpha}\right)^{\frac{m}{c}}\\
\end{split}
\end{equation}
\end{proof}

\begin{lemma}\label{lem:sm1} [in supplementary proof]
For $c>1$ and $m,\frac{m}{c}\in \mathbbm{Z}_+$,
$$\sum_{l_1=0}^{m/c} e^{-\alpha l_1}\binom{\frac{m}{c}}{l_1}\binom{m-\frac{m}{c}}{\frac{m}{c}-l_1} \leq \binom{m}{\frac{m}{c}}\left(1-\frac{1}{c}+\frac{1}{ce^\alpha}\right)^{\frac{m}{c}}$$
\end{lemma}
\begin{proof}
It is clear that left side of "$\leq$" is the $\frac{m}{c}$-th order term of polynomial $(1+e^{-\alpha}x)^{\frac{m}{c}}\cdot(1+x)^{m-\frac{m}{c}}$, and the right side of "$\leq$" is the $\frac{m}{c}$-th order term of polynomial $\left[1+\left(1-\frac{1}{c}+\frac{1}{ce^{\alpha}}\right)x\right]^{m}$.
Intuitively, we know the first inequality is always no greater than the second one. Then, we prove this claim is also true for any order terms of $x$.
\begin{lemma} [in supplementary proof]
For $a>b>0$ and $l\in \mathbbm{Z}_+$, it is true for any $i$-th order terms that,
\begin{equation}\nonumber
\begin{split}
&i\text{-th order term of}\left[(1+ax)(1+bx)^{l-1}\right]\\
\leq\;& i\text{-th order term of}\left(1+\frac{a}{l}x+\frac{l-1}{l}bx\right)^l
\end{split}
\end{equation}
\end{lemma}
\begin{proof}
We first check the polynomial at the left side of "$\leq$"
\begin{equation}\nonumber
\begin{split}
&i\text{-th order term of}\left(1+\frac{a}{l}x+\frac{l-1}{l}bx\right)^l\\
=\;& ax\binom{l}{i}\left[\left(\frac{a}{l}+\frac{l-1}{l}b\right)x\right]^i\\
=\;& \left[\binom{l-1}{i-1}+\binom{l-1}{i}\right]\left(\frac{a}{l}+\frac{l-1}{l}b\right)^ix^i\\
\end{split}
\end{equation}
For the other polynomial,
\begin{equation}\nonumber
\begin{split}
&i\text{-th order term of}\left[(1+ax)(1+bx)^{l-1}\right]\\
=\;& ax\binom{l-1}{i-1}(bx)^{i-1} + \binom{l-1}{i}(bx)^{i}\\
=\;& \left[a\binom{l-1}{i-1}+b\binom{l-1}{i}\right]b^{i-1}x^i\\
\leq\;& \left[\binom{l-1}{i-1}+\binom{l-1}{i}\right]ab^{i-1}x^i\\
\leq\;& \left[\binom{l-1}{i-1}+\binom{l-1}{i}\right]\left(\frac{a}{l}+\frac{l-1}{l}b\right)^ix^i\\
=\;& i\text{-th order term of}\left(1+\frac{a}{l}x+\frac{l-1}{l}bx\right)^l\\
\end{split}
\end{equation}

\end{proof}
By letting $a =1$, $b=e^{-\alpha}$ and $l=\frac{m}{c}+1$ for the lemma above, we knoe it is true for any $i$-th order terms that,\\
\begin{equation}\nonumber
\begin{split}
&i\text{-th order term of}\left[(1+x)(1+e^{-\alpha}x)^{\frac{m}{c}}\right]\\
\leq\;& i\text{-th order term of}\left(1+\frac{1}{\frac{m}{c}+1}x+\frac{\frac{m}{c}}{\frac{m}{c}+1}e^{-\alpha}x\right)^{\frac{m}{c}+1}
\end{split}
\end{equation}
and Lemma \ref{lem:sm1} follows by induction.
\end{proof}

\subsection{Correctness proof of corrected nearest neighbor algorithm}
\subsubsection{1D case}

We first prove the monotonicity of $\E[D(x_i,x_j)]$ in the neighborhood of $x_i$.

\begin{theorem}\label{the:CP1}
For $y_1,\cdots, y_m, x_k \in[0,1]$, any $1>\varepsilon>0$ , $x_i = x_j-\varepsilon$, $y_1,\cdots,y_m\sim^{i.i.d.}\mathcal{D}_Y$, $x_k\sim \mathcal{D}_X$ such that $\frac{\max{d_Y}}{\min{d_Y}} = c_Y$ and $\frac{\max{d_X}}{\min{d_X}} = c_X$,  we have,
\begin{equation}\nonumber
\E[D(x_i,x_j)]\leq c_Y^2x_i(1-x_i)\varepsilon + O(\varepsilon^2)
\end{equation}
where $d_X$ and $d_Y$ are the probability density function of $D_X$ and $X_Y$ independently.
\end{theorem}
}

==> old_wrong_lower_bound.tex <==
\begin{theorem}\label{thm:wrong} Let $\cald_X$ be a uniform distribution on $[0, 1]$, $x_{n + 1} \leq 0.25$, and $O_{n + 1} = [m]$. Let $x \in [0, 1]$ be an arbitrary agent and $R_x$ be the ranking of the agent $x$ (which is a random variable conditioned on $x$). We have: 
\begin{itemize}[noitemsep,topsep=0pt]
\setlength{\itemsep}{-2pt}
\setlength{\parskip}{-2pt}
\setlength{\parsep}{0pt}
\item When $x_{n + 1} \leq 0.25$:
\begin{equation}
x^* = \arg \min_x \E_{Y} \left[\nkt(R_{n +1}, R_x)\right]\} = 0
\end{equation}
\item When $x_{n + 1} \geq 0.75$: 
\begin{equation}
x^* = \arg \min_x \E_{Y} \left[\nkt(R_{n +1}, R_x)\right]\} = 1.
\end{equation}
\end{itemize}
\end{theorem}
\vspace{-4mm}
{\color{blue} Q: made the itemize and following itemize tight.}
This theorem shows that even we have full observation of the rankings of agent $n + 1$, and $X$ is sufficiently large and dense, the nearest neighbor for $x_{n + 1}$ (under the normalized Kendal-Tau distance) is $x = 0$ ($x = 1$) for any $x_{n + 1} < 0.25$ ($x_{n + 1} > 0.75$), \ie this method is always biased regardless of the dataset size. 

{\color{red}ZL in this proof, where did we use the fact that $x_{n + 1} < 0.25$?}

{\color{red}Ao: we used the fact of $x_{n + 1} < 0.25$ to give a bound to $x_{n+1}$ and $x$. We further use those bounds when bounding $\Delta$ terms}

\begin{proof}[Proof of Theorem~\ref{thm:wrong}] We shall show only the first part of the theorem. The second part can be analyzed in a similar fashion. Because $\calf(x) \equiv  \E_Y[\nkt(R_{n + 1}, R_x) \mid x_{n + 1}]$ is a function of $x$ and is continuous, we use $d\calf(x)/dx$ to characterize the minimal point $x$. Specifically, we shall show that $d \calf(x)/dx > 0$ for all $x \in [0, 1]$, which means the function is minimized when $x = 0$. 

We next calculate $d\calf(x)/dx$. Let $p_x(y_1, y_2) = \Pr[y_1 \succ_x y_2 \mid y_1, y_2]$ and $p_{n + 1}(y_1, y_2) = \Pr[y_1 \succ_{n + 1}y_2 \mid y_1, y_2]$. When the context is clear, we will write $p_x$ and $p_{n + 1}$ instead. We have
$$\E[\nkt(R_x, R_{n + 1}) \mid x_{n + 1}] = \E_{y_1, y_2}\left[\E[\nkt(R_x, R_{n + 1} \mid y_1, y_2, x_{n + 1}] \right].$$
Next, we have 
$$\E_{y_1, y_2}[\nkt(R_x, R_{n + 1})\mid y_1, y_2, x_{n + 1}]  = p_x(1-p_{n + 1}) + p_{n + 1}(1-p_x).$$

Therefore, we have 
$$\frac{d\calf(x)}{dx} = \E_{y_1, y_2}\left[(1-2p_{n + 1})\frac{dp_x}{dx}\right].$$
Let $\deltax = |y_2 - x| - |y_1 - x|$ and $\deltan = |y_2 - x_{n + 1}| - |y_1 - x_{n + }1|$. We have 
\begin{eqnarray*}
& & \E_{y_1, y_2}\left[(1-2p_{n + 1})\frac{dp_x}{dx}\right] \\
& = & \E_{y_1, y_2}\left[\frac{e^{-\deltan} - 1}{e^{-\deltan} + 1}\cdot \frac{\sign(y_1 - x) - \sign(y_2 - x)}{4\cosh^2(\deltax/2) }\right] \\
& = & \E_{y_1 < y_2}\left[\frac{e^{-\deltan} - 1}{e^{-\deltan} + 1}\cdot \frac{\sign(y_1 - x) - \sign(y_2 - x)}{4\cosh^2(\deltax/2) }\right] 
\end{eqnarray*}
The last equation holds because $y_1$ and $y_2$ are symmetric. 

To simplify the notation, let $\Phi(y_1, y_2, x, x_n + 1) = \frac{e^{-\deltan} - 1}{e^{-\deltan} + 1}\cdot \frac{\sign(y_1 - x) - \sign(y_2 - x)}{4\cosh^2(\deltax/2)}$ (sometimes we simply use $\Phi$ when the context is clear). Define the following events: 
\begin{itemize}[noitemsep,topsep=0pt]
\setlength{\itemsep}{0pt}
\setlength{\parskip}{0pt}
\setlength{\parsep}{0pt}
\item $\cale_0$: when $y_2 \geq y_1 \geq x$. 
\item $\cale_1$: when $y_1 \leq x$ and $y_2 \geq 2 x_{n + 1}$. 
\item $\cale_2$: when $y_1 \leq x$ and $x \leq y_2 \leq 2x_{n + 1} - x$. 
\item $\cale_3$: when $y_1 \leq x$ and $2x_{n + 1} - x \leq y_2 \leq 2x_{n + 1}$. 
\end{itemize}
We have 
\begin{equation}
\E_{y_1 \leq y_2}[\Phi \mid x_{n + 1}] = \sum_{0 \leq i \leq 3}\E_{y_1 \leq y_2}[\Phi\mid \cale_i]\Pr[\cale_i]. 
\end{equation}
First note that $\E_{y_1 \leq y_2}[\Phi \mid \cale_0] = 0$ because 
$$\sign(y_1 - x) - \sign(y_2 - x)\mid \cale_0 = 0.$$

Next, we will compute each of $\E_{y_1 \leq y_2}[\Phi \mid \cale_i]$ for $i = 1,2,3$. Before proceeding, we state useful properties of an important function: 

{\color{red} we need to highlight where the fact below is used.}
\begin{fact}\label{fact:wrong}
Let $g(x) = \frac{e^{-x}-1}{e^{-x}}$, we have 
\begin{itemize}[noitemsep,topsep=0pt]
\setlength{\itemsep}{0pt}
\setlength{\parskip}{0pt}
\setlength{\parsep}{0pt}
\item $g(x) = - g(-x)$. 
\item $g''(x) \cdot g(x) \geq 0$. 
\item $|g(x)| \leq \frac 1 2 g(x)$. 
\end{itemize}
\end{fact}
\vspace{-4mm}
\mypara{Case 1. $\E[\Phi \mid \cale_1]$. } Observe that $\deltax \in [2x_{n + 1}-2x, 1 - x]$, $\sign(y_1-x)-\sign(y_2-x) = -2$ and $\deltan > 0$. Therefore, $\E[\deltan \mid \cale_1] = \frac{1-x}{2} - x_{n + 1}$. We have
\begin{eqnarray*}
& & \E_{y_1 < y_2}[\Phi\mid \cald_1] \\
& \geq & \E_{y_1 < y_2}\left[g(\deltan)\frac{-2}{4\cosh^2(\frac 1 2)} \mid \cald_1\right] \\
& \geq & \frac{-2}{4\cosh^2\left(\frac{1}{2}\right)} \\
& & \times \E_{y_1,y_2}\left[\left.\Delta_{1,2}^{(n+1)}g(1)+\left(1-\Delta_{1,2}^{(n+1)}\right)g(0)\right| \cale_1 \right] \\
& \geq & \frac{2e(e-1)}{\left(1+e\right)^3}\cdot\left(\frac{1+x_i}{2}-x_{n+1}\right)
\end{eqnarray*}
The second "$\geq$" comes from the 2nd item in Fact \ref{fact:wrong}, which shows the concavity of $g(\cdot)$

\mypara{Case 2. $\E[\Phi \mid \cale_2]$.} We have $\deltan < 0$, $\sign(y_1-x)-\sign(y_2-x) = -2$ and $\deltax \in [-x, 2x_{n + 1} - x]$. Therefore, $\E[\deltan \mid \cale_2] = -\frac{x_{n + 1}}{2}$. 
With some algebra manipulation, we have 
\begin{eqnarray*}
& & \E[\Phi \mid \cale_2] \\
& = & \E_{y_1 < y_2}\left[g(\deltan \frac{-2}{4\cosh^2(\deltax/2)}\right] \\
& \geq & \E_{y_1,y_2}\left[g\left(\deltan\right)\cdot\left.\frac{-2}{\left(e^{0}+e^{0}\right)^2}\right| \cale_2 \right] \\
& \geq^* &  -\frac{1}{2}\,\mathbbm{E}_{y_1,y_2}\left[\left.\frac{1}{2}{\deltan}\right| \cale_2 \right]\\
& \geq & -\frac{x_{n + 1}}{8}. 
\end{eqnarray*}
$\geq^*$ comes from the 3rd item in  Fact \ref{fact:wrong}.

\mypara{Case 3. $\E[\Phi \mid \cale_3]$.} We have $\deltax \in [x_{n + 1} - 3x, 2x_{n + 1}]$, $\sign(y_1-x)-\sign(y_2-x) = -2$ and $\E[\deltan\mid \cale_3] = 0$. Let $y'_1 = 2x_{n + 1} - y_1$ and $y'_2 = 2x_{n + 1} - y_2$. Note that we also have $y'_1 \leq x$ and $(2x_{n + 1} - x \leq y'_2 \leq 2 x_{n + 1}$. Therefore, 
\begin{eqnarray*}
& & \E[\Phi \mid \cale_3] \\
& = & \E_{y_1 < y_2}[\Phi(y_1, y_2, x, x_{n + 1}) + \Phi(y'_1, y'_2, x, x_{n + 1}\mid \cale_3 \deltan > 0] \\
& =^* & \E_{y_1 < y_2}\left[g(\deltan) \left(\frac{-2}{4\cosh^2(\deltax/2)} - \frac{2}{4\cosh^2(\deltaxp/2)}\right)\right] 
\\
& \geq & \E_{y_1 < y_2}\left[g(\deltan) \left(\frac{-2}{4\cosh^2(\deltan/2)} - \frac{2}{4\cosh^2(0)}\right)\right] \\
& \geq & \left(\frac{1}{4\cosh^2(x_{n + 1}/2)} - \frac{1}{4\cosh^2(0)}\right)x_{n + 1} \\
\end{eqnarray*}
$=^*$ used the 1st item in  Fact \ref{fact:wrong}.
Now we can see that 
\begin{eqnarray*}
& & \E[\Phi] \\
& = & \sum_{1 \leq i \leq 3}\E_{y_1 < y_2}\E[\Phi \mid \cale_i]\Pr[\cale_i \mid y_1 < y_2]\\
& \geq & \frac{2e(e-1)}{(1+e)^3}\left(\frac{1+x}{2} - x_{n + 1}\right)\cdot x(1-2x_{n + 1}) \\
& & - \frac{x_{n + 1}}{8}x(2x_{n + 1} - 2x) + \left(\frac{1}{4\cosh^2(x_{n + 1}/2)} - \frac{1}{4\cosh^2(0)}\right)x_{n + 1}x^2 \\
& \geq & x_i\left[\frac{2e(e-1)}{\left(1+e\right)^3}\cdot\frac{1}{4}\cdot\frac{1}{2}-\frac{1}{8}\cdot\frac{1}{4}\cdot\frac{1}{2}-0.0155\cdot\frac{1}{4}\cdot\frac{1}{4}\right] \\
& \geq & 0. 
\end{eqnarray*}
Equality holds if and only if $x = 0$. Therefore, $\calf(x)$ is minimized at $x = 0$. 
\end{proof}


{\color{red} ZL's edit on 20180206 ends here. }
\begin{proof}



\begin{lemma}
For $D_Y = \text{Uniform}[0,1]$, $x_i\in [x_{n+1},\,1-x_{n+1}]$ and $x_{n+1}\leq 0.25$, we have,
$$\mathbbm{E}_{Y}\left[\nkt(R_{n +1}, R_i)\right] \geq \mathbbm{E}_{Y}\left[\nkt(R_{n +1}, R_{n+1'})\right]$$
Where $R_{n+1'}$ is the ranking of $x_{n+1}'$, another agent at the same position as $x_{n+1}$ in latent space.
\end{lemma}
\begin{proof}
We similarly define $p_{n+1'} = \mathbbm{P}[y_1\succ_{n+1'} y_2]$ and it is clear that $p_{n+1'} = p_{n+1}$. Thus, we have,\\
$$\mathbbm{E}_{Y}\left[\nkt(R_{n +1}, R_{n+1}')\right] = \mathbbm{E}_{y_1,y_2}\left[2p_{n+1}(1-p_{n+1})\right]\;\text{and}$$
$$\mathbbm{E}_{Y}\left[\nkt(R_{n +1}, R_i)\right] = \mathbbm{E}_{y_1,y_2}\left[p_{n+1}+(1-2p_{n+1})p_i\right]$$
For any $y_1,y_2 \in [0,x_i+x_{n+1}]$, we define $y_1' = x_i+x_{n+1}-y_1$ and $y_2' = x_i+x_{n+1}-y_2$. It is also clear that $D_Y(y_1)\cdot D_Y(y_2) = D_Y(y_1')\cdot D_Y(y_2')$. If we assume $y_1\geq y_2$, we always have $y_1'<y_2'$. We further define $p_{n+1}' = \mathbbm{P}[y_1'\succ_{n+1} y_2']$ and $p_{i}' = \mathbbm{P}[y_1'\succ_{i} y_2']$. It is clear that $p_{n+1}' = p_i$ and $p_{i}' = p_{n+1}$,and we have,
\begin{equation}\nonumber
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{n+1}')\Big|y_1,y_2\leq x_i+x_{n+1}\right]\\
=\;& \mathbbm{E}_{y_1,y_2}\left[p_{n+1}(1-p_{n+1})+p_i(1-p_i)\Big|x_i+x_{n+1}\geq y_2\geq y_1\right]
\end{split}
\end{equation}
\begin{equation}\nonumber
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{i})\Big|y_1,y_2\leq x_i+x_{n+1}\right]\\
=\;& \mathbbm{E}_{y_1,y_2}\left[p_{n+1}+(1-2p_{n+1})p_i\Big|x_i+x_{n+1}\geq y_2\geq y_1\right]
\end{split}
\end{equation}
Then, we always have,
\begin{equation}\nonumber
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{i})\Big|y_1,y_2\leq x_i+x_{n+1}\right] -\\
& \mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{n+1}')\Big|y_1,y_2\leq x_i+x_{n+1}\right]\\
=\;&\mathbbm{E}_{y_1,y_2}\left[p_{n+1}^2+p_i^2-2p_ip_{n+1}\Big|x_i+x_{n+1}\geq y_2\geq y_1\right]\\
\geq\;& 0\\
\end{split}
\end{equation}
For the case that $y_1\leq x_i+x_{n+1}\leq y_2$ or $y_2\leq x_i+x_{n+1}\leq y_1$, we know that this two subcases are equivalent because of the symmetry of $y_1$ and $y_2$. So, for $y_1\leq x_i+x_{n+1}\leq y_2$, we have,
\begin{equation}\nonumber
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{i})\Big|y_1\leq x_i+x_{n+1}\leq y_2\right] - \\
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{n+1'})\Big|y_1\leq x_i+x_{n+1}\leq y_2\right]\\
=\;&\mathbbm{E}_{y_1,y_2}\left[p_i(1-p_{n+1})+p_{n+1}(1-p_i)-2p_{n+1}(1-p_{n+1})\Big|\right.\\
&\;\;\;\;\;\;\;\;\;\;\;\left.y_1\leq x_i+x_{n+1}\leq y_2\right]\\
=\;&\mathbbm{E}_{y_1,y_2}\left[(p_i-p_{n+1})(1-2p_{n+1})\Big|y_1\leq x_i+x_{n+1}\leq y_2\right]\\
\end{split}
\end{equation}
Because $|y_1-x_{n+1}|\geq|y_2-x_{n+1}|$ for $y_1\leq x_i+x_{n+1}\leq y_2$, $1-2p_{n+1} \leq 0$ is always true. Then,
\begin{equation}\nonumber
\begin{split}
&p_{n+1} = \frac{e^{-|x_{n+1}-y_1|}}{e^{-|x_{n+1}-y_1|}+e^{-|y_2-x_{n+1}|}}\\
=\;&\frac{e^{-\left(|x_{n+1}-y_1|-|x_i-x_{n+1}|\right)}}{e^{-\left(|x_{n+1}-y_1|-|x_i-x_{n+1}|\right)}+e^{-|y_2-x_i|}}\\
\geq\;& \frac{e^{-|x_i-y_1|}}{e^{-|x_i-y_1|}+e^{-|y_2-x_i|}} = p_i
\end{split}
\end{equation}
Thus, we have
\begin{equation}\label{eqn:case1}
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{i})-\nkt(R_{n +1}, R_{n+1'})\Big|\right.\\
&\left.y_1\leq x_i+x_{n+1}\leq y_2\right] \geq 0
\end{split}
\end{equation}
\begin{equation}\label{eqn:case2}
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{i})-\nkt(R_{n +1}, R_{n+1'})\Big|\right.\\
&\left.y_2\leq x_i+x_{n+1}\leq y_1\right] \geq 0
\end{split}
\end{equation}
We also know that
\begin{equation}\label{eqn:case3}
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{i})-\nkt(R_{n +1}, R_{n+1'})\Big|\right.\\
&\left.y_1,y_2\geq x_i+x_{n+1}\right] = 0
\end{split}
\end{equation}
And Lemma 3.4 follows by combining (\ref{eqn:case1}), (\ref{eqn:case2}) and (\ref{eqn:case3}).
\end{proof}
$x_{n+1}\leq 0.25$ part of Theorem 3.1 follows by combining all lemmas above in this section and $x_{n+1}\geq 0.75$ part follows by symmetry of $x_{n+1}\leq 0.25$ part.
\end{proof}

==> partial_obs.tex <==
\section{Text for the partial observation model}

over a subset $O_i \subseteq [m]$ of alternatives. The ranking $R_i$ is generated by the following two-step procedure: \emph{(i)} Using the \emph{Plackett-Luce model}~\cite{Plackett75:Analysis,Luce77:Choice}. Let $j_1, \dots j_m$ be a random permutation of $[m]$, we have 
\begin{equation}\label{eqn:pleq}
\Pr\left[y_{j_1}\succ_i \cdots\succ_i y_{j_m}\right] = \prod_{\ell=1}^m\dfrac{u(x_i,y_{j_l})}{\sum_{k=1}^m u(x_i,y_{j_k})}. 
\end{equation}
\emph{(ii)} Random sampling. After agent $i$ determines its ranking, it will random select a subset $O_i$ and reveals his/her ranking over $O_i$. We shall let agent $i$'s ranking over $O_i$ be $R_i$ and its ranking over $[m]$ (\ie including those we have not observed) be $\tilde R_i$. 


==> residual.tex <==
\subsection{Notations}

$m$: number of alternatives (items).\\
\indent $n$: number of agents (users).\\
\indent $x_i$: the $i^{th}$ agent, we also abuse this notation $x_i$ to represent $x_i$'s latent feature vector in $\mathbbm{R}^{d}$.\\
\indent $y_j$: the $j^{th}$ alternative, we also abuse this notation $y_j$ to represent $y_j$'s latent feature vector in $\mathbbm{R}^{d}$.\\


Each agent $i$ observes a subset $O_i \subseteq [m]$ of alternatives and give a ranking over $O_i$. 
 
Since an agent $i$ may not rank all alternatives, let $R_i$ denote agent $i$'s ranking over $O_i\subseteq Y$. The feature vectors and the utility functions are not observed. We further assume that features of agents and alternatives are i.i.d.~generated from fixed but unknown distributions, denoted by $\cald_X$ and $\cald_Y$, respectively ($d_X$ and $d_Y$ to denote the corresponding probability density functions).

\mypara{Utility function.} Throughout this paper, we focus on a utility function that depends on only the Euclidean distance between $x_i$ and $y_j$:
$$u(x_i, y_j) = e^{-\|x_i - y_j\|}$$

\mypara{Distributions $\cald_X$ and $\cald_Y$.} For exposition purpose, we further make simplifying assumption that $d = 1$ and have $\frac{\max\left(d_X\right)}{\min\left(d_X\right)} \leq c_X$ and $\frac{\max\left(d_Y\right)}{\min\left(d_Y\right)} \leq c_Y$. We briefly comment on the $d = 2$ case in {\color{red} Section X}. Our model is the same as Katz-Samuels \etal so far.


\emph{Randomized setting.} Each agent's ranking is generated randomly such that alternatives with higher utilities will be more preferred with higher probability according to the celebrated {\em Plackett-Luce model}~\cite{Plackett75:Analysis,Luce77:Choice}. More precisely, for $\{j_1,\ldots, j_m\}=\{1,\ldots, m\}$,
\begin{equation}\label{eqn:pleq}
\mathbbm{P}\left[y_{j_1}\succ_i \cdots\succ_i y_{j_m}\right] = \prod_{l=1}^m\dfrac{\exp(u(x_i,y_{j_l}))}{\sum_{k=l}^m\exp(u(x_i,y_{j_k}))}
\end{equation}
In this formula, the first term can be seen as the probability to choose $y_{j_1}$ among all alternatives; the second term can be seen as the probability to choose $y_{j_2}$ among $\{y_{j_k}:k\ge 2\}$, etc.

\begin{remark} While we focus on only a specific form of the utility function, and assume $\cald_X$ and $\cald_Y$ are near-uniform in 1-dimensional space, most of our results can be generalized to other utility functions in possibly high dimensional space. We will discuss about the generalizations in {\color{red} Section X}.
\end{remark}

==> wrong_lower_bound_v0208.tex <==
\section{Harmful nearest neighbors}\label{sec:wronglower}
This section explains why Algorithm~\label{alg:classical} is incorrect under the Plackett-Luce random utility model. 
Let $\bar R_i$ be the ground-truth ranking of agent $i$, \ie the $j$-th element in $R_{n + 1}$ is the $j$-th largest value of the set $\{u(x_{i}, y_j)\}$.

\mypara{Design ``intuition'' for \wrongalgo.} \wrongalgo was thought to be correct because of the following intuitions: (i) if $x_i$ and $x_{j}$ are close, then $\bar R_i$ and $\bar R_{j}$ are also close, and (ii) if $\bar R_i$ and $\bar R_{j}$ are close, their ``realizations'' $R_i$ and $R_{j}$ are also going to be close. Therefore, one may think when $x_j$ minimizes $\kt(R_i, R_j)$ for large $n$ and $m$, it also minimizes $\kt(\bar R_i, \bar R_j)$.  

Intuition (i) is theoretically-grounded (see~\cite{SamuelsS17}). The key problematic ``intuition'' is that $\kt(\bar R_i, \bar R_j)$ and $\kt(R_i, R_j)$ \emph{do not} have monotone relationship (\ie an increase in $\kt(\bar R_i, \bar R_j)$ does not necessarily imply an increase in $\kt(R_i, R_j)$, and vice versa).

\begin{example}\label{example:simplewrong} Let $y_1 = 0.4$ and $y_2 = 0.7$. Let $x_1 = 0.5$. Consider the following two optimization problems:
\begin{equation}\label{eqn:minbarkt}
x_2 = \arg \min_{x_2} \{ \kt(\bar R_1, \bar R_2)\}.
\end{equation}
\begin{equation}\label{eqn:minkt}
x_2 = \arg \min_{x_2} \{\E [\kt(R_1,  R_2)]\}
\end{equation} We can see that the structures of these two optimization problems are very different. In (\ref{eqn:minbarkt}), the optimal solution set is $(-\infty, 0.55)$ (\ie any $x_2$ inside $(-\infty, 0.55)$ works). But for (\ref{eqn:minkt}), the optimal solution set is $(-\infty, -0.4)$ (\eg $x_1$ itself would be an optimal solution in (\ref{eqn:minbarkt}) but it is not an optimal solution in (\ref{eqn:minkt}).
\end{example}

\myparab{Interpreting the result.} 
We need to solve (\ref{eqn:minbarkt}) to find nearest neighbors but the objective of \wrongalgo is closer to (\ref{eqn:minkt}). Specifically, 
consider a scenario in which there are only two alternatives $\{y_1,y_2\}$ but $n$ is sufficiently large. Example~\ref{example:simplewrong} shows that $\arg \min_{x_2} \{\E [\kt(R_1,  R_2)]\}$ is far away from $x_1$. Because $n$ is sufficiently large, we have $\arg \min_{x_2 \in [0,1]} \{\E [\kt( R_1,  R_2)]\} \approx \arg \min_{x_2 \in X} \{\E [\kt(R_1, R_2)]\}$. The right side of the approximation resembles the nearest-neighbor approximation (\ie $\min_{x_2 \in X} \{\kt( R_1,  R_2)\}$) because $\kt(R_1, R_2)$ converges to its expectation for large $m$. Therefore, \wrongalgo solves (\ref{eqn:minkt}) which could be very different from solving (\ref{eqn:minkt}). 

This observation can be used to build a more general negative example. 

\begin{theorem}\label{thm:wrong} Let $\cald_X$ be a uniform distribution on $[0, 1]$, and $O_{n + 1} = [m]$. Let $x \in [0, 1]$ be an arbitrary agent and $R_x$ be the ranking of the agent $x$ (which is a random variable conditioned on $x$). We have:
\begin{itemize}[noitemsep,topsep=0pt]
\setlength{\itemsep}{-2pt}
\setlength{\parskip}{-2pt}
\setlength{\parsep}{0pt}
\item When $x_{n + 1} \leq 0.25$:
\begin{equation}
x^* = \arg \min_x \E_{Y} \left[\nkt(R_{n +1}, R_x)\right]\} = 0
\end{equation}
\item When $x_{n + 1} \geq 0.75$:
\begin{equation}
x^* = \arg \min_x \E_{Y} \left[\nkt(R_{n +1}, R_x)\right]\} = 1.
\end{equation}
\end{itemize}
\end{theorem}
\vspace{-4mm}
{\color{blue} Q: made the itemize and following itemize tight.}

{\color{red}ZL in this proof, where did we use the fact that $x_{n + 1} < 0.25$?}

{\color{red}Ao: we used the fact of $x_{n + 1} < 0.25$ to give a bound to $x_{n+1}$ and $x$. We further use those bounds when bounding $\Delta$ terms}

\begin{proof}[Proof of Theorem~\ref{thm:wrong}] We shall show only the first part of the theorem. The second part can be shown by symmetry.

\begin{lemma}\label{lemma:wrong1}
Let $\cald_X$ be a uniform distribution on $[0, 1]$, $x_{n + 1} \leq 0.25$, and $O_{n + 1} = [m]$. Let $x \in [0, x_{n+1}]$ be an arbitrary agent and $R_x$ be the ranking of the agent $x$ (which is a random variable conditioned on $x$). We have:
$$x^* = \arg \min_{x\leq x_{n+1}} \E_{Y} \left[\nkt(R_{n +1}, R_x)\right]\} = 0$$
\end{lemma}

\begin{proof}
Because $\calf(x) \equiv  \E_Y[\nkt(R_{n + 1}, R_x) \mid x_{n + 1}]$ is a function of $x$ and is continuous, we use $d\calf(x)/dx$ to characterize the minimal point $x$. Specifically, we shall show that $d \calf(x)/dx > 0$ for all $x \in [0, 1]$, which means the function is minimized when $x = 0$.

We next calculate $d\calf(x)/dx$. Let $p_x(y_1, y_2) = \Pr[y_1 \succ_x y_2 \mid y_1, y_2]$ and $p_{n + 1}(y_1, y_2) = \Pr[y_1 \succ_{n + 1}y_2 \mid y_1, y_2]$. When the context is clear, we will write $p_x$ and $p_{n + 1}$ instead. We have
\begin{eqnarray*}
& &\E[\nkt(R_x, R_{n + 1}) \mid x_{n + 1}]\\
& = &  \E_{y_1, y_2}\left[\E[\nkt(R_x, R_{n + 1}) \mid y_1, y_2, x_{n + 1}] \right]\\
& = & \E_{y_1, y_2}[p_x(1-p_{n + 1}) + p_{n + 1}(1-p_x)]
\end{eqnarray*}

Therefore, we have
$$\frac{d\calf(x)}{dx} = \E_{y_1, y_2}\left[(1-2p_{n + 1})\frac{dp_x}{dx}\right].$$
Let $\deltax = |y_2 - x| - |y_1 - x|$ and $\deltan = |y_2 - x_{n + 1}| - |y_1 - x_{n + }1|$. We have
\begin{eqnarray*}
& & \E_{y_1, y_2}\left[(1-2p_{n + 1})\frac{dp_x}{dx}\right] \\
& = & \E_{y_1, y_2}\left[\frac{e^{-\deltan} - 1}{e^{-\deltan} + 1}\cdot \frac{\sign(y_1 - x) - \sign(y_2 - x)}{4\cosh^2(\deltax/2) }\right] \\
& = & \E_{y_1 < y_2}\left[\frac{e^{-\deltan} - 1}{e^{-\deltan} + 1}\cdot \frac{\sign(y_1 - x) - \sign(y_2 - x)}{4\cosh^2(\deltax/2) }\right]
\end{eqnarray*}
The last equation holds because $y_1$ and $y_2$ are symmetric.

To simplify the notation, let $\Phi(y_1, y_2, x, x_n + 1) = \frac{e^{-\deltan} - 1}{e^{-\deltan} + 1}\cdot \frac{\sign(y_1 - x) - \sign(y_2 - x)}{4\cosh^2(\deltax/2)}$ (sometimes we simply use $\Phi$ when the context is clear). Define the following events:
\begin{itemize}[noitemsep,topsep=0pt]
\setlength{\itemsep}{0pt}
\setlength{\parskip}{0pt}
\setlength{\parsep}{0pt}
\item $\cale_0$: when $y_2 \geq y_1 \geq x$.
\item $\cale_1$: when $y_1 \leq x$ and $y_2 \geq 2 x_{n + 1}$.
\item $\cale_2$: when $y_1 \leq x$ and $x \leq y_2 \leq 2x_{n + 1} - x$.
\item $\cale_3$: when $y_1 \leq x$ and $2x_{n + 1} - x \leq y_2 \leq 2x_{n + 1}$.
\end{itemize}
We have
\begin{equation}
\E_{y_1 \leq y_2}[\Phi \mid x_{n + 1}] = \sum_{0 \leq i \leq 3}\E_{y_1 \leq y_2}[\Phi\mid \cale_i]\Pr[\cale_i].
\end{equation}
First note that $\E_{y_1 \leq y_2}[\Phi \mid \cale_0] = 0$ because
$$\sign(y_1 - x) - \sign(y_2 - x)\mid \cale_0 = 0.$$

Next, we will compute each of $\E_{y_1 \leq y_2}[\Phi \mid \cale_i]$ for $i = 1,2,3$. Before proceeding, we state useful properties of an important function:

{\color{red} we need to highlight where the fact below is used.}
\begin{fact}\label{fact:wrong}
Let $g(x) = \frac{e^{-x}-1}{e^{-x}}$, we have
\begin{itemize}[noitemsep,topsep=0pt]
\setlength{\itemsep}{0pt}
\setlength{\parskip}{0pt}
\setlength{\parsep}{0pt}
\item $g(x) = - g(-x)$.
\item $g''(x) \cdot g(x) \geq 0$.
\item $|g(x)| \leq \frac 1 2 g(x)$.
\end{itemize}
\end{fact}
\vspace{-4mm}
\mypara{Case 1. $\E[\Phi \mid \cale_1]$. } Observe that $\deltax \in [2x_{n + 1}-2x, 1 - x]$, $\sign(y_1-x)-\sign(y_2-x) = -2$ and $\deltan > 0$. Therefore, $\E[\deltan \mid \cale_1] = \frac{1-x}{2} - x_{n + 1}$. We have
\begin{eqnarray*}
& & \E_{y_1 < y_2}[\Phi\mid \cald_1] \\
& \geq & \E_{y_1 < y_2}\left[g(\deltan)\frac{-2}{4\cosh^2(\frac 1 2)} \mid \cald_1\right] \\
& \geq & \frac{-2}{4\cosh^2\left(\frac{1}{2}\right)} \\
& & \times \E_{y_1,y_2}\left[\left.\Delta_{1,2}^{(n+1)}g(1)+\left(1-\Delta_{1,2}^{(n+1)}\right)g(0)\right| \cale_1 \right] \\
& \geq & \frac{2e(e-1)}{\left(1+e\right)^3}\cdot\left(\frac{1+x_i}{2}-x_{n+1}\right)
\end{eqnarray*}
The second "$\geq$" comes from the 2nd item in Fact \ref{fact:wrong}, which shows the concavity of $g(\cdot)$

\mypara{Case 2. $\E[\Phi \mid \cale_2]$.} We have $\deltan < 0$, $\sign(y_1-x)-\sign(y_2-x) = -2$ and $\deltax \in [-x, 2x_{n + 1} - x]$. Therefore, $\E[\deltan \mid \cale_2] = -\frac{x_{n + 1}}{2}$.
With some algebra manipulation, we have
\begin{eqnarray*}
& & \E[\Phi \mid \cale_2] \\
& = & \E_{y_1 < y_2}\left[g(\deltan \frac{-2}{4\cosh^2(\deltax/2)}\right] \\
& \geq & \E_{y_1,y_2}\left[g\left(\deltan\right)\cdot\left.\frac{-2}{\left(e^{0}+e^{0}\right)^2}\right| \cale_2 \right] \\
& \geq^* &  -\frac{1}{2}\,\mathbbm{E}_{y_1,y_2}\left[\left.\frac{1}{2}{\deltan}\right| \cale_2 \right]\\
& \geq & -\frac{x_{n + 1}}{8}.
\end{eqnarray*}
$\geq^*$ comes from the 3rd item in  Fact \ref{fact:wrong}.

\mypara{Case 3. $\E[\Phi \mid \cale_3]$.} We have $\deltax \in [x_{n + 1} - 3x, 2x_{n + 1}]$, $\sign(y_1-x)-\sign(y_2-x) = -2$ and $\E[\deltan\mid \cale_3] = 0$. Let $y'_1 = 2x_{n + 1} - y_1$ and $y'_2 = 2x_{n + 1} - y_2$. Note that we also have $y'_1 \leq x$ and $(2x_{n + 1} - x \leq y'_2 \leq 2 x_{n + 1}$. Therefore,
\begin{eqnarray*}
& & \E[\Phi \mid \cale_3] \\
& = & \E_{y_1 < y_2}[\Phi(y_1, y_2, x, x_{n + 1}) + \Phi(y'_1, y'_2, x, x_{n + 1}\mid \cale_3 \deltan > 0] \\
& =^* & \E_{y_1 < y_2}\left[g(\deltan) \left(\frac{-2}{4\cosh^2(\deltax/2)} - \frac{2}{4\cosh^2(\deltaxp/2)}\right)\right]
\\
& \geq & \E_{y_1 < y_2}\left[g(\deltan)\left(\frac{-2}{4\cosh^2(\deltan/2)} - \frac{2}{4\cosh^2(0)}\right)\right] \\
& \geq & \left(\frac{1}{4\cosh^2(x_{n + 1}/2)} - \frac{1}{4\cosh^2(0)}\right)x_{n + 1} \\
\end{eqnarray*}
$=^*$ used the 1st item in  Fact \ref{fact:wrong}.

Now, by applying $0\leq x\leq x_{n+1} \leq \frac{1}{4}$, we can see that,
\begin{eqnarray*}
& & \E[\Phi] \\
& = & \sum_{1 \leq i \leq 3}\E_{y_1 < y_2}\E[\Phi \mid \cale_i]\Pr[\cale_i \mid y_1 < y_2]\\
& \geq & \frac{2e(e-1)}{(1+e)^3}\left(\frac{1+x}{2} - x_{n + 1}\right)\cdot x(1-2x_{n + 1}) \\
& & - \frac{x_{n + 1}}{8}x(2x_{n + 1} - 2x)\\
& & + \left(\frac{1}{4\cosh^2(x_{n + 1}/2)} - \frac{1}{4\cosh^2(0)}\right)x_{n + 1}x^2 \\
& \geq & x_i\left[\frac{2e(e-1)}{\left(1+e\right)^3}\cdot\frac{1}{4}\cdot\frac{1}{2}-\frac{1}{8}\cdot\frac{1}{4}\cdot\frac{1}{2}-0.0155\cdot\frac{1}{4}\cdot\frac{1}{4}\right] \\
& \geq & 0.
\end{eqnarray*}
Equality sign holds if and only if $x = 0$. Therefore, $\calf(x)$ is minimized at $x = 0$.
\end{proof}



{\color{red} ZL's edit on 20180206 ends here. }

Using similar analysis tool as Lemma \ref{lemma:wrong1}, we can get the following lemma for $x\in[1-x_{n+1},1]$

\begin{lemma}\label{lemma:wrong2}
Let $\cald_X$ be a uniform distribution on $[0, 1]$, $x_{n + 1} \leq 0.25$, and $O_{n + 1} = [m]$. Let $x \in [1-x_{n+1},1]$ be an arbitrary agent and $R_x$ be the ranking of the agent $x$ (which is a random variable conditioned on $x$). We have:
$$x^* = \arg \min_{x\geq 1-x_{n+1}} \E_{Y} \left[\nkt(R_{n +1}, R_x)\right]\} = 1-x_{n+1}$$
\end{lemma}

We further discuss the case for $x\in[1-x_{n+1},1]$

\begin{lemma}\label{lemma:wrong3}
Let $\cald_X$ be a uniform distribution on $[0, 1]$, $x_{n + 1} \leq 0.25$, and $O_{n + 1} = [m]$. Let $x \in [x_{n+1},1-x_{n+1}]$ be an arbitrary agent and $R_x$ be the ranking of the agent $x$ (which is a random variable conditioned on $x$). We have:
$$x^* = \arg \min_{x \in [x_{n+1},1-x_{n+1}]} \E_{Y} \left[\nkt(R_{n +1}, R_x)\right]\} = x_{n+1}$$
\end{lemma}
\begin{proof}
Similar to the proof of Lemma \ref{lemma:wrong1}, we have,
$$\mathbbm{E}_{Y}\left[\nkt(R_{n +1}, R_x)\right] = \mathbbm{E}_{y_1,y_2}\left[p_{n+1}+(1-2p_{n+1})p_x\right]$$
and specially,
\begin{equation}\nonumber
\begin{split}
&\mathbbm{E}_{Y}\left[\nkt(R_{n +1}, R_x)\mid x = x_{n+1}\right]\\
=\;& \mathbbm{E}_{y_1,y_2}\left[2p_{n+1}(1-p_{n+1})\right]
\end{split}
\end{equation}
To simplify the notation, define the following events for Lemma \ref{lemma:wrong3}:
\begin{itemize}[noitemsep,topsep=0pt]
\setlength{\itemsep}{0pt}
\setlength{\parskip}{0pt}
\setlength{\parsep}{0pt}
\item $\cale_0$: when $y_1,y_2 \geq x+x_{n+1}$.
\item $\cale_1$: when $y_1,y_2 \leq x+x_{n+1}$.
\item $\cale_2$: when $y_1 \geq x+x_{n+1} \geq y_2$ or $y_2 \geq x+x_{n+1} \geq y_1$
\end{itemize}
\mypara{Case 0. $\E[\nkt(R_{n +1}, R_x) \mid \cale_0]$. }

Using the same tool as used in Case 0 of Lemma \ref{lemma:wrong1}, we have,
\begin{equation}\label{eqn:case1}
\E[\nkt(R_{n +1}, R_x) \mid \cale_0] = 0
\end{equation}

\mypara{Case 1. $\E[\nkt(R_{n +1}, R_x) \mid \cale_1]$. }


For any $y_1,y_2 \in [0,x+x_{n+1}]$, we define $y_1' = x+x_{n+1}-y_1$ and $y_2' = x+x_{n+1}-y_2$. If we assume $y_1\geq y_2$, we always have $y_1'\leq y_2'$. By further defining $p_{n+1}' = \mathbbm{P}[y_1'\succ_{n+1} y_2']$ and $p_{x}' = \mathbbm{P}[y_1'\succ_{x} y_2']$. We have $p_{n+1}' = p_x$ and $p_{x}' = p_{n+1}$ and
\begin{equation}\label{equ:x}
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_x)\Big|\cale_1\right]\\
=\;& \mathbbm{E}_{y_1,y_2}\left[p_{n+1}+(1-2p_{n+1})p_x\Big|\cale_1\right]\\
=\;& \mathbbm{E}_{y_1\leq y_2}\left[p_{n+1}+(1-2p_{n+1})p_x \right.\\
&\;\;\;\;\;\;\;\;\;\;\;\left.+ p_{n+1}'+(1-2p_{n+1}')p_x'\Big|\cale_1\right]\\
=\;& 2\mathbbm{E}_{y_1\leq y_2}\left[p_{n+1}+(1-2p_{n+1})p_x\Big|\cale_1\right]\\
\end{split}
\end{equation}
Similarly, we have,
\begin{equation}\label{equ:n}
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_x)\Big|\cale_1,\,x = x_{n+1}\right]\\
=\;& \mathbbm{E}_{y_1, y_2}\left[2p_{n+1}(1-p_{n+1})\Big|\cale_1\right]\\
=\;& \mathbbm{E}_{y_1\leq y_2}\left[2p_{n+1}(1-p_{n+1})+ 2p_{n+1}'(1-p_{n+1}')\Big|\cale_1\right]\\
=\;& 2\mathbbm{E}_{y_1\leq y_2}\left[p_{n+1}(1-p_{n+1})+p_{x}(1-p_{x})\Big|\cale_1\right]\\
\end{split}
\end{equation}
Combining Equation \ref{equ:x} and \ref{equ:n}, we have:\\
\begin{equation}\label{eqn:case2}
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_x)\Big|\cale_1\right]-\\
& \mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_x)\Big|\cale_1,\,x = x_{n+1}\right]\\
=\;& 2\mathbbm{E}_{y_1\leq y_2}\left[p_{n+1}+(1-2p_{n+1})p_x\Big|\cale_1\right]-\\
& 2\mathbbm{E}_{y_1\leq y_2}\left[p_{n+1}(1-p_{n+1})+p_{x}(1-p_{x})\Big|\cale_1\right]\\
=\;& 2\mathbbm{E}_{y_1\leq y_2}\left[p_{n+1}^2-2p_{x}p_{n+1}+p_{x}^2\Big|\cale_1\right]\\
\geq\;&0
\end{split}
\end{equation}


\mypara{Case 2. $\E[\nkt(R_{n +1}, R_x) \mid \cale_2]$. }

It is clear that $y_1 \geq x+x_{n+1} \geq y_2$ and $y_2 \geq x+x_{n+1} \geq y_1$ are equivalent because of the symmetry between $y_1$ and $y_2$. So, we only study the event $\cale_{2.1} = y_2 \geq x+x_{n+1} \geq y_1$, 
\begin{equation}\nonumber
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{x})\Big|\cale_{2.1}\right] - \\
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{x})\Big|\cale_{2.1},\,x = x_{n+1}\right]\\
=\;&\mathbbm{E}_{y_1,y_2}\left[p_x(1-p_{n+1})+p_{n+1}(1-p_x)-2p_{n+1}(1-p_{n+1})\Big|\cale_{2.1}\right]\\
=\;&\mathbbm{E}_{y_1,y_2}\left[(p_x-p_{n+1})(1-2p_{n+1})\Big|\cale_{2.1}\right]\\
\end{split}
\end{equation}

Because $|y_1-x_{n+1}|\leq|y_2-x_{n+1}|$ when $y_1\leq x_i+x_{n+1}\leq y_2$, we always have $1-2p_{n+1} \leq 0$ . Then,
\begin{equation}\nonumber
\begin{split}
p_{n+1} =\;& \frac{e^{-|x_{n+1}-y_1|}}{e^{-|x_{n+1}-y_1|}+e^{-|y_2-x_{n+1}|}}\\
=\;&\frac{e^{-\left(|x_{n+1}-y_1|-|x-x_{n+1}|\right)}}{e^{-\left(|x_{n+1}-y_1|-|x-x_{n+1}|\right)}+e^{-|y_2-x|}}\\
\geq\;& \frac{e^{-|x-y_1|}}{e^{-|x-y_1|}+e^{-|y_2-x_i|}} = p_x
\end{split}
\end{equation}
Thus, we have
\begin{equation}\label{eqn:case3}
\begin{split}
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{x})\Big|\cale_{2}\right] - \\
&\mathbbm{E}_{y_1,y_2}\left[\nkt(R_{n +1}, R_{x})\Big|\cale_{2},\,x = x_{n+1}\right]\geq\;0
\end{split}
\end{equation}

And Lemma 3.4 follows by combining (\ref{eqn:case1}), (\ref{eqn:case2}) and (\ref{eqn:case3}).
\end{proof}
$x_{n+1}\leq 0.25$ part of Theorem 3.1 follows by combining Lemma \ref{lemma:wrong1}- \ref{lemma:wrong3} and $x_{n+1}\geq 0.75$ part follows by symmetry.
\end{proof}
